Node Max-Cut and Computing Equilibria in Linear Weighted Congestion Games

In this work, we seek a more refined understanding of the complexity of local optimum computation for Max-Cut and pure Nash equilibrium (PNE) computation for congestion games with weighted players and linear latency functions. We show that computing a PNE of linear weighted congestion games is PLS-complete either for very restricted strategy spaces, namely when player strategies are paths on a series-parallel network with a single origin and destination, or for very restricted latency functions, namely when the latency on each resource is equal to the congestion. Our results reveal a remarkable gap regarding the complexity of PNE in congestion games with weighted and unweighted players, since in case of unweighted players, a PNE can be easily computed by either a simple greedy algorithm (for series-parallel networks) or any better response dynamics (when the latency is equal to the congestion). For the latter of the results above, we need to show first that computing a local optimum of a natural restriction of Max-Cut, which we call \emph{Node-Max-Cut}, is PLS-complete. In Node-Max-Cut, the input graph is vertex-weighted and the weight of each edge is equal to the product of the weights of its endpoints. Due to the very restricted nature of Node-Max-Cut, the reduction requires a careful combination of new gadgets with ideas and techniques from previous work. We also show how to compute efficiently a $(1+\eps)$-approximate equilibrium for Node-Max-Cut, if the number of different vertex weights is constant.

==> BeforeICALP/TODO.tex <==
@patsilinakos

fix augmentation figure nodes (A->B in figure 8 and (x+1) index in figure 7)

Fix architecture figures to have bolded circles in muiplt nodes (Like T)

indices in the feedback gadgets


simmetric prasinakia

==> BeforeICALP/colors.tex <==
 \definecolor{1}{rgb}{0.368417, 0.506779, 0.709798}
 \definecolor{2}{rgb}{0.880722, 0.611041, 0.142051}
 \definecolor{3}{rgb}{0.560181, 0.691569, 0.194885}
 \definecolor{4}{rgb}{0.922526, 0.385626, 0.209179}
 \definecolor{5}{rgb}{0.528488, 0.470624, 0.701351}
 \definecolor{6}{rgb}{0.772079, 0.431554, 0.102387}
 \definecolor{7}{rgb}{0.363898, 0.618501, 0.782349}
 \definecolor{8}{rgb}{1, 0.75, 0}
 \definecolor{9}{rgb}{0.647624, 0.37816, 0.614037}
 \definecolor{10}{rgb}{0.571589, 0.586483, 0.}
 \definecolor{11}{rgb}{0.915, 0.3325, 0.2125}
 \definecolor{12}{rgb}{0.40082222609352647, 0.5220066643438841, 0.85}
 \definecolor{13}{rgb}{0.9728288904374106, 0.621644452187053, 0.07336199581899142}
 \definecolor{14}{rgb}{0.736782672705901, 0.358, 0.5030266573755369}
 \definecolor{15}{rgb}{0.28026441037696703, 0.715, 0.4292089322474965}


==> BeforeICALP/macrosOLD.tex <==
% MACROS.
\newcommand{\GR}{\selectlanguage{greek}}
\newcommand{\EN}{\selectlanguage{english}}
%display style in FRAC
\newcommand\ddfrac[2]{\frac{\displaystyle #1}{\displaystyle #2}}


\newcommand{\lp}{\left}
\newcommand{\rp}{\right}
\newcommand{\mrm}[1]{\mathrm{#1}}
\newcommand{\mbb}[1]{\mathbb{#1}}
\newcommand{\mcal}[1]{\mathcal{#1}}
\newcommand{\mfrak}[1]{\mathfrak{#1}}
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\maj}{maj}

%Tikz crap.
\newcommand*{\equal}{=}
\newcommand*{\comma}{,}

% Asymptotic Notation.
\newcommand{\bigOh}[1]{O\lp(#1\rp)}
\newcommand{\smalloh}[1]{o\lp(#1\rp)}
\newcommand{\bigOmega}[1]{\Omega\lp(#1\rp)}
\newcommand{\smallomega}[1]{\omega\lp(#1\rp)}
\newcommand{\poly}{\mrm{poly}}

% Standard sets
\newcommand{\R}{\bm{\mrm{R}}}
\newcommand{\N}{\bm{\mrm{N}}}
\newcommand{\Q}{\bm{\mrm{Q}}}
\newcommand{\Z}{\bm{\mrm{Z}}}

% Constants.
\newcommand{\me}{\mathrm{e}}

% Analysis.
\def\d{\mrm{d}}
\newcommand\Ball[2]{\mcal{B}\lp(#1, #2 \rp)}
\newcommand\norm[2]{\| #2 \|_{#1}}

% Functions.
\newcommand{\tr}{\mathrm{tr}}
\newcommand{\1}[1]{\bm{1}{\left[#1\right]}}
\newcommand{\Real}[1]{\mathrm{Re}\lp(#1\rp)}
\newcommand{\Imag}[1]{\mathrm{Im}\lp(#1\rp)}
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}

% Distances & Probability.
\newcommand{\Normal}[2]{\mcal{N}\lp(#1,#2\rp)}
\newcommand{\DNormal}[2]{\mrm{DN}\lp(#1,#2\rp)}
\newcommand{\GBD}{\mrm{GBD}}
\newcommand{\PBD}{\mrm{PBD}}
\newcommand{\Bin}{\mrm{Bin}}
\newcommand{\Pois}{\mrm{Pois}}
\newcommand{\Distr}{\mathcal{L}}
\newcommand{\Unif}{\mrm{U}}

% \newcommand{\GBD}[1][]{
%   \def\ArgI{{#1}}%
%   \GBDRelay
% }
% \newcommand{\GBDRelay}[1]{
%   \mrm{GBD}\lp( \ArgI, #2 \rp)
% }

\newcommand{\NormalPDF}[3]
{
  \frac{1}{\sqrt{2 \pi} #2} \me^{-\frac{(#3 - #1)^2}{2 {#2}^2}}
}
\newcommand{\erf}[1]{\mrm{erf}\lp(#1\rp)}
\newcommand{\erfc}[1]{\mrm{erfc}\lp(#1\rp)}

\newcommand{\Prob}[1]{\bm{\mrm{P}}\lp[#1\rp]}

\newcommand{\Exp}[1][]{
  \def\ArgI{#1}%
  \ExpRelay
}
\newcommand{\ExpRelay}[1]{
  \bm{\mrm{E}}_{\ArgI} \lp[ #1 \rp]
}

\newcommand{\Expnew}[2]{
  \bm{\mrm{E}}_{#1} \lp[ #2 \rp]
}


\newcommand{\Var}[1]{\bm{\mrm{V}}\lp[#1\rp]}
\newcommand{\Cov}[2]{\mrm{Cov}\lp[#1, #2\rp]}
\newcommand{\Kurt}[1]{\mrm{Kurt}\lp[#1 \rp]}

\newcommand{\fdiv}[3]{D_{#1} \lp(#2\|#3\rp)}
\newcommand{\dkl}[2]{D_{\mrm{kl}} \lp(#1\|#2\rp) }
\newcommand{\dtv}[2]{d_{\mrm{tv}} \lp(#1, #2\rp) }
\newcommand{\dhel}[2]{d_{\mrm{hel}} \lp(#1, #2\rp) }
\newcommand{\dkol}[2]{d_{\mrm{kol}} \lp(#1, #2\rp) }

% minimax risk
\newcommand{\minimax}[1]{\mfrak{M}_{#1}}

\newcommand{\h}[1]{\hat{#1}}

% PBD powers specific macros.
\def\eps{\varepsilon}
\def\p{\hat{p}}
\def\q{\hat{q}}

\def\reals{\bm{\mrm{R}}}
\def\nats{\mathbb{N}}
\def\D{\mathcal{D}}

\def\P{\mathcal{P}}
\def\p{\hat{p}}
\def\q{\hat{q}}
\newcommand{\err}[1]{\mbox{\rm err}\left(#1\right)}


% other.

\newcommand{\sline}[1]{\textcolor{#1}{\linethickness{.5mm}\line(1,0){15}} }

% Ident in algorithmic.
\newlength\myindent
\setlength\myindent{2em}
\newcommand\bindent{%
  \begingroup
  \setlength{\itemindent}{\myindent}
  \addtolength{\algorithmicindent}{\myindent}
}
\newcommand\eindent{\endgroup}


%LLNCS repeat theorem.
\newcommand{\repeattheorem}[1]{%
  \begingroup
  \renewcommand{\thetheorem}{\ref{#1}}%
  \expandafter\expandafter\expandafter\theorem
  \csname reptheorem@#1\endcsname
  \endtheorem
  \endgroup
}
\NewEnviron{reptheorem}[1]{%
  \global\expandafter\xdef\csname reptheorem@#1\endcsname{%
    \unexpanded\expandafter{\BODY}%
  }%
  \expandafter\theorem\BODY\unskip\label{#1}\endtheorem
}


\newcommand{\repeatlemma}[1]{%
  \begingroup
  \renewcommand{\thelemma}{\ref{#1}}%
  \expandafter\expandafter\expandafter\protect\lemma
  \csname replemma@#1\endcsname
  \protect\endlemma
  \endgroup
}

\NewEnviron{replemma}[1]{%
  \global\expandafter\xdef\csname replemma@#1\endcsname{%
    \unexpanded\expandafter{\BODY}%
  }%
  \expandafter\lemma\BODY\unskip\label{#1}\endlemma
}


\makeatletter
\newcommand*{\inlineequation}[2][]{%
  \begingroup
    % Put \refstepcounter at the beginning, because
    % package `hyperref' sets the anchor here.
    \refstepcounter{equation}%
    \ifx\\#1\\%
    \else
      \label{#1}%
    \fi
    % prevent line breaks inside equation
    \relpenalty=10000 %
    \binoppenalty=10000 %
    \ensuremath{%
      % \displaystyle % larger fractions, ...
      #2%
    }%
    \qquad \@eqnnum
  \endgroup
}
\makeatother


==> BeforeICALP/packagesOLD.tex <==
\usepackage[margin=1in]{geometry}
\usepackage[T1]{fontenc}
\usepackage{lmodern}
\usepackage{microtype}
%\usepackage{ifthen}
%\usepackage{mathptmx}
\usepackage{bbm}
\usepackage[titletoc]{appendix}
\DeclareMathAlphabet{\pazocal}{OMS}{zplm}{m}{n}
\usepackage[iso-8859-7]{inputenc}
%\usepackage[english,greek]{babel}
% fonts.
%\usepackage{fontspec}

% linespread looks better for mathpazo
% \linespread{1.05}
% \usepackage[sc]{mathpazo}
% \usepackage{kpfonts}
% \usepackage[boldsans]{ccfonts}
% \usepackage{beton}
% \usepackage{kurier}

% \usepackage{eulervm}
% \usepackage[euler-digits]{eulervm}

% \usepackage{concrete}
% \usepackage{sectsty}
% \allsectionsfont{\mdseries}
% \renewcommand{\bfdefault}{sbc}

% \setmainfont{Linux Libertine}

% \usepackage{ntheorem}

% \usepackage{newpxtext}

% allows for indexgeneration
\usepackage{makeidx}

\usepackage{amsfonts}
\usepackage{amsmath}
\usepackage{thmtools}
\usepackage{amsthm}
\usepackage{amssymb}
\usepackage{mathtools}
\usepackage{thm-restate}
% \usepackage{algorithm}
\usepackage{algorithm, algorithmic}
% Theorem Environments.
% Comment out for llncs.
% \usepackage{amsthm}
% \renewcommand\qedsymbol{$\blacksquare$}

 \newtheorem{definition}{Definition}
 \newtheorem{theorem}{Theorem}
 \newtheorem{lemma}{Lemma}
 \newtheorem{corollary}{Corollary}
% \newtheorem{claim}{Claim}
  \newtheorem*{question}{Question}
% \newtheorem{theorem}{Theorem}
% \newtheorem{definition}{Definition}
 \newtheorem{assumption}{Assumption}
 \newtheorem{remark}{Remark}
 \newtheorem{example}{Example}
\usepackage{hyperref}
\hypersetup{
  colorlinks = true,
  urlcolor = {blue},
  citecolor = {blue}
}

\usepackage{textcomp}
\usepackage{csquotes}

\usepackage{booktabs}
\usepackage[scale=2]{ccicons}
\usepackage{graphicx}

\usepackage{pgfplots}
\usepgfplotslibrary{dateplot}
\usepackage{color}

\usepackage{listings, color}
\definecolor{green}{rgb}{0,0.5,0}
\definecolor{gray}{rgb}{0.4,0.4,0.4}
\definecolor{lblue}{rgb}{0.9,0.9,1}
\definecolor{red}{rgb}{0.9,0,0}
\definecolor{blue}{rgb}{0.6,0,0.6}

% \DeclareSymbolFont{matha}{OML}{txmi}{m}{it}% txfonts
% \DeclareMathSymbol{\varv}{\mathord}{matha}{118}

% bold vectors
\usepackage{bm}

% mathbb numbers
\usepackage{dsfont}

% mathlarger
\usepackage{relsize}

%\usepackage{algorithmic}
  % \usepackage[noend]{algpseudocode}
  % \makeatletter
  % \def\BState{\State\hskip-\ALG@thistlm}
  % \makeatother

\lstset{
  backgroundcolor=\color{lblue},
  basicstyle=\scriptsize\ttfamily,
  breaklines=true,
  columns=fullflexible,
  commentstyle=\color{gray},
  keywordstyle=\color{blue},
  stringstyle=\color{red},
  identifierstyle=\color{black},
  language=haskell,
  % numbers=left,
  % numberstyle=\scriptsize,
  % numbersep=5pt,
  showstringspaces=false
}

\usepackage{subcaption}

% Tikz.
\usepackage{tikz}
\usetikzlibrary{arrows}
\usetikzlibrary{arrows.meta}
\tikzstyle{line}=[draw]

%LLNCShit for repeated theorems.
\usepackage{environ}


==> intro.tex <==
\section{Introduction}

Among the strongest notions in Game Theory is that of a Nash equilibrium. Although its existence is always guaranteed in normal form games if mixed strategies are allowed, its computation is more often inefficient than efficient. This is true even if the game admits a potential function and any improving step by a player reduces the value of the potential, in which case we additionally know that a Nash equilibrium on \emph{pure strategies} always exists. In such \emph{potential games}, a pure Nash equilibrium (or simply equilibrium) can be computed by letting the players one by one play their best response, %(on pure strategies) 
until they eventually reach an equilibrium, which of course may take exponentially many steps. In a sense, the described \emph{best response} dynamics is equivalent to searching for an extremum by doing local improving steps. 

 Polynomial Local Search  (PLS) is a complexity class defined by  Johnson et al. \cite{JPY88} to capture the difficulty of certain search problems. It consists of problems that admit local search heuristics that are guaranteed to converge to a local optimum, like the problem of finding an equilibrium in potential games described above. There are many natural complete problems for PLS (see, e.g., \cite{MA10} for a survey) many of which are or can be regarded as the problem of computing an equilibrium in a potential game. That said, PLS fully captures the difficulty of such problems. Complete problems particularly relevant to this work are \lmc{} and \cf{} which we will describe later, and the problem of computing an equilibrium in Congestion Games.
 

 Congestion Games (CGs) are one of the most widely studied classes of games in Algorithmic Game Theory. In CGs players compete over resources trying to minimize their costs. More precisely, there exists a set of resources $E$ and the strategy of each selfish agent is a subset of
 resources $s_i \in 2^E$ that she selects. The cost of each agent $i$ for a given strategy vector $s = (s_i,s_{-i})$ is the
 cumulative congestion on the each resources that she selects to use. More precisely, the cost of agent $i$ is  
 $C_i(x_i,x_{-i}) = \sum_{e \in s_i} \ell_e(x_e)$, where $x_e$ is the number of agents participating in resource $e$ and $\ell_e(x)$ is latency function of resource $e$. Usually agents are not allowed to select any subset of resources. The permitted subsets 
 may differ from agent to agent and
 are denoted by $S_i \subseteq 2^E$. The case where all the $S_i$'s are the same set is referred as \emph{Symmetric CGs}.
  
Congestion Games are of interest
not only due to their obvious connection to resource sharing in networks and distributed
systems with selfish users, but also due to their unique game theoretic properties. Congestion games are potential games, i.e., there exists a potential function mapping each strategy profile to a real number, $\Phi(s) = \sum_{e \in E} \sum_{x=1}^{x_e} \ell_e(x)$, so that whenever an agent changes her strategy to reduce her cost, the potential function decreases. The latter not only provides a proof of existence of an equilibrium, but also provides a pseudo-polynomial algorithm for computing one (best response dynamics). Unfortunately a polynomial algorithm for computing an equilibrium is highly unlikely to exist since this problem was proven to be PLS-complete \cite{FPT04}.



Although computing an equilibrium in general CGs is PLS-complete, there are important special cases in which an equilibrium can be computed efficiently. A notable example concerns computing an equilibrium in single-commodity Network CGs. In this type of games, there exists a network with  latency functions on its edges together with an  origin node $o$ and a target node $d$. The strategy space of each agent is the set of $o-d$ paths. Fabrikant et al. \cite{FPT04} provide an efficient algorithm for computing an equilibrium, which is based on solving a suitable min-cost flow problem. Another interesting special case where approximate equilibrium can be efficiently computed by approximate best response dynamics concerns a general class of Symmetric CGs \cite{CS07}.



An important generalization of CGs is that of Weighted CGs where the players are weighted,  putting a different load on the resources they choose. Since Weighted CGs are a generalization of  CGs computing an equilibrium is a harder task.
Many recent works study algorithms for computing an approximate 
equilibrium in general CGs (see the related work section). The reason for this is twofold: At first, computing an exact equilibrium is for sure PLS-hard and, second, Weighted CGs with general latency functions are not potential games, meaning that exact equilibria may not even exist. 

Our work is motivated by the fact that the forementioned results do not provide a vivid picture of the differences  between weighted and  unweighted CGs, since in the general setting both
are hard. In order get a better understanding of these differnces
we examine the computational hardness of computing equilibria in Weighted CGs for the  cases in which an equilibrium can be computed efficiently for their unweighted counterparts.

This work deals with the problem of computing equilibria in Weighted Network CGs with linear latency functions on the links of the network. The choice of linear functions ensures the existence of a potential function \cite{FKS05}, rendering the problem of computing equilibrium in PLS. We prove PLS-completeness
both for the single-commodity, i.e., all agents want to travel from a common origin $o$ to a common destination $d$, and to the multi-commodity case where each agent $i$ has a different pair $(o_i,d_i)$ of origin-destination nodes. Obviously, the second type of games is a generalization of the first. The reason that two different PLS-reductions are provided is that in the single-commodity case we study a more general set of latency functions by allowing them to have exponential coefficients, 
while in the multi-commodity case all the linear latency functions have coefficient $1$. 
We highlight that in the case of equally weighted players both equilibria can be efficiently computed. In the first case via a min-cost flow computation, while in the second using \emph{best response dynamics}, which converges in a polynomial number of steps.




\smallskip\noindent
\textbf{Contribution.}
First we show that computing an equilibrium even in single-commodity Weighted Network CGs with linear latency functions is PLS-complete (Theorem \ref{thm:sepaPLShard}).
Our result reveals a huge gap between the weighted and the unweighted case for this class of
CGs, since Papadimitriou et al.  \cite{FPT04} designed a polynomial time algorithm for computing equilibrium in single-commodity (unweighted) Network CGs with general increasing latency functions. For the proof we reduce from \lmc{}, one of the most significant PLS-complete problems. We highlight that our reduction not only uses simple linear latency functions (i.e., of the form $\ell(x)=ax$), but also
the network topology used for our reduction is that of series-parallel networks.

Trying to further understand the differences between  weighted and unweighted CGs,
we turn our attention to the case where all resources/links have the identity latency function (i.e., for all e: $\ell_e(x)=x$) and only the players' weights are allowed to be exponential. The reason for this choice is that an equilibrium in general (unweighted) CGs with this type of functions can be efficiently computed using best response dynamics. 
We manage to show that computing an equilibrium even in multi-commodity Weighted Network CGs where all links have the identity function is PLS-complete (Theorem \ref{thm:mutiPLS}). For the above reduction, none of the already  known PLS-complete problems seemed suitable, since their intrinsic difficulty  lies in the interactions between players, while the complexity of our problem stems from the weights of the players themselves.
This should not
be a surprise, since in general CGs with this type of latency functions and equally weighted agents an equilibrium can be efficiently computed. Thus, in order to prove Theorem \ref{thm:mutiPLS} we introduce as an intermediate problem a simple variant of \lmc{} that we call \lnmc{}.

\lnmc{} is a  natural special case of \lmc{} where the weights of the edges are related in a specific way. Namely, each node has a positive weight and 
the weight of each edge  is the product of the weights of its endpoints. As in  \lmc{}, the goal is to find a maximal cut of the edges, i.e., a partition of the nodes so that the total weight
of the edges traversing the cut cannot be increased by moving any single node from one side of the partition to the other. Interestingly enough,
\lnmc{} is suitable for the reduction 
we want due to the weights on the nodes, while at the same time it is expressive enough to be PLS-complete.

Our major technical contribution is proving that \lnmc{} is PLS-complete. To establish its PLS-hardness we did not use a problem that lies on any of the ``reduction paths'' departing from \lnmc{}, as this seemd unnatural since \lnmc{} is a very restrictive special case of \lmc{}. Instead we turned to the very first problem proved to be PLS-complete, i.e., \cf{}. 
 Note that a similar problem to \lnmc{}, that of computing a local optimum of an unweighted graph, was shown by Sch\:affer and Yannakakis \cite{SY91} to be P-complete. 


In \lnmc{} it is very crucial  that nodes see other nodes  in the same way. More precisely, any two nodes see the same weight on any third node, in contrast to \lmc{} where the weights on the edges may be distributed so that nodes see common neighboring nodes differently. This lack of freedom is very restrictive in many places of the PLS-completeness of \lmc{} but we manage to overcome it via more sophisticated ideas combined with gadgets already used  by Els\:asser and Tscheuschner \cite{ET11} and   Gairing and Savani \cite{GS10}. Our technical work, though, is difficult to be explained at a high level and so, instead of getting  into its details here, we highlight it at the end of Section \ref{sec:nMCoverview}. The ideas used there can be adapted to simplify proofs in existing work \cite{ET11,GS10}  and we conjecture that they also can be used to prove hardness of approximation results for Weighted Network CGs with ``natural'' latency functions, thus  complementing the existing results for the unweighted case \cite{SV08}.


\smallskip\noindent
\textbf{Related Work.}
While  Weighted CGs do not always possess exact equilibria, there is a large amount of literature concerning cases of Weighted CGs
in which exact or approximate equilibria can be efficiently computed. Fotakis et al. \cite{FKS05} show that in the case of linear latencies the existence of an equilibrium is guaranteed by a potential argument.  Even-Dar et al. \cite{EKM03} study different best-response schemes for weighted congestion games in series of parallel links. In case of identity latency functions it was proven that the max-weight priority best response policy reaches equilibrium in linear steps.  Goldberg \cite{G04} analyzes the convergence time to a Nash equilibrium of a randomized local search distributed protocol  in the case of series-parallel links with different capacities.
 Gairing et al. \cite{GLMM04} present a polynomial algorithm   for computing Nash equilibrium in the restricted case of  parallel links, i.e., each agent can select a subset of the overall links.  Caragiannis et al. \cite{CFGS11} and Giannakopouloset al. \cite{GNS18}  design efficient algorithms for computing approximate equilibria in Weighted CGs with polynomial latencies. More algorithmic results for approximate equilibria in Weighted CGs are provided by 
Fanelli and Moscardelli  \cite{FM09} and Feldotto et al.  \cite{FGKS17}.

To capture the difficulty of local search problems, Johnson et al. \cite{JPY88} define the class PLS that consists of problems admitting a
polynomial time algorithm for computing a better neighbor solution. They prove that all such problems can be reduced to a general optimization problem named \cf{}. Later, Sch\"aeffer and Yannakakis \cite{SY91} used \cf{}
to prove that \lmc{} is PLS-complete. \lmc{}
searches for a cut in an edge-weighted undirected graph such that the cumulative weight of the edges
traversing the cut cannot be increased by changing the set of any single node. It was used to establish  the PLS-completeness
of computing equilibria in general unweighted CGs \cite{FPT04}. In the same paper PLS-completeness of computing an equilibrium for multi-commodity Network CGs was proven through a very involved proof. Ackermann et al.  \cite{ARV08} provide a much simpler PLS-completeness proof of the previous result via a reduction from \lmc{}. 

From a technical point of view,
most related to our work are the PLS-completeness results for variants of \lmc{} by Els\"asser and Tscheuschner \cite{ET11} and  Gairing and Savani \cite{GS10} who adapted the original construction of Sch\"affer and Yannakakis \cite{SY91}. Gairing and Savani \cite{GS10} establish PLS-completeness of computing a Nash equilibrium in hedonic games, while Els\"asser and Tscheuschner \cite{ET11}  show that \lmc{} remains PLS-complete even if the underlying graph has nodes of degree at most five.  Skopalik and V\"ocking  \cite{SV08} proved that it PLS-complete to compute an $\alpha$-approximate Nash equilibrium in general unweighted congestion games.




\smallskip\noindent
\textbf{Organization.} 
The paper is organized as follows.  In Section~\ref{sec:wcgsOverview} we present proof sketches for the hardness results regarding computing  equilibria in single-commodity Weighted CGs %(with exponential coefficients)
and multi-commodity Weighted CGs. %with the identity function on all  links. 
In Section~\ref{sec:nMCoverview}, we give an overall presentation of the way our \lnmc{} PLS-reduction %from \cf{} to for
works, while omitting certain details. The fully detailed proofs are deferred to the appendix, in sections \ref{s:CG}  and \ref{s:MC}, respectively.

%Also somewhere write: main difference for the special case of \lnmc{} that nodes see other nodes  in the same way, in contrast to \lmc{} where the weights on the value edges may be distributed so that nodes see common neighboring nodes differently. This lack of freedom is very restrictive in many places of the PLS-completeness of \lmc{} but we manage to overcome it via more sophisticated ideas combined with gadgets in [CITE TWO PAPERS].  

==> nMCoverview.tex <==
\section{PLS-completeness of \lnmc{}}%Overview of the Reduction}
\label{sec:nMCoverview}
In this section we present the proof of Theorem~\ref{t:main_max_cut}
which states that \lnmc{} is \emph{PLS}-complete. As discussed in the preliminaries, \lnmc{} is in PLS and thus it remains to prove its PLS-hardness. To do so, we reduce \cf{} to it. We remind that an instance of \lnmc{}
is composed by an undirected graph $G(N,A)$, 
and the weights of each vertex $i\in N$, $w_i \geq 0$. Given a circuit $\text{\emph{C}}$ of the \cf{}, we construct an instance of \lnmc{} such as
from any Nash Equilibrium we can compute in polynomial time
a locally maximal solution for the \cf{} problem.

Given a circuit \emph{C} of \cf{}, the vertex-weighted graph that we construct is a combination of different gadgets which themselves might be seen as smaller instances of \lnmc{}. These gadgets have different goals but what each of them intuitively does is receiving  some information to some of its vertices, the ``input'' vertices,  and transforming it while carrying it through its internal part towards the ``output'' vertices. These input and output vertices  are the vertices through which the different gadgets are connected. The connections are not always simple and we will later go into more detail on how these connections are done.

\begin{figure}[h]
    \centering
    \includegraphics[scale = 0.5]{Architecture.jpg}
    \caption{The high level construction of the \nmc{} instance. Note that rectangles represent gadgets that will be defined below, circles represent vertices that take part in multiple gadgets, and bolded black circles represent a set of \emph(n) such vertices. The computation gadgets are represented by $C_A$ and $C_B$.}
\label{f:construction}
\end{figure}

Our construction 
follows
a \emph{flip-flop architecture} that has been previously used for reductions from  \cf{} to  \lmc{} 
and some of
its variants \cite{SY91,GS10,ET11}, but requires more sophisticated implementations in many of its gadgets, since we deal with the special case of \lnmc. The most important differences and our major technical contributions are summarized at the end of the section.
The constructed instance is  presented at a high level in Figure~\ref{f:construction}.
Next, we discuss the role of each separate gadget. The 
exact construction of each separate gadget is presented in the respective section of the appendix.


For a given circuit \emph{C} of the \cf{} with \emph{n} input gates and \emph{m} output gates, we first construct the \emph{Circuit Computing} gadgets $\text{\emph{C}}\ell$ (for $\ell=A,B$). These gadgets are instances of \lnmc{} that simulate \emph{C} in the following sense: $\text{\emph{I}}_\ell$ is a set of \emph{n} vertices whose values correspond  to an ``input string'' of \emph{C}. $\text{\emph{Val}}_\ell$ is a set of \emph{m} vertices whose values correspond to the output of circuit \emph{C} with input string $\text{\emph{I}}_\ell$.
$\text{\emph{Next}}\ell$ is a set of \emph{n} vertices that represent a neighbor string of $\text{\emph{I}}_\ell$ with greater output value in \emph{C}. 
More precisely, if the ``input'' string defined by the values of $\text{\emph{I}}_\ell$, has a neighbor solution (Hamming distance \emph{1}) with \emph{strictly} greater cost then the values of the \emph{n} vertices in $\text{\emph{Next}}\ell$ correspond to this neighbor string. In case such a neighbor string does not exist (which means that $\text{\emph{I}}_\ell$ is an optimal solution to  \cf{}) the values of the vertices in $\text{\emph{Next}}\ell$ equal $\text{\emph{I}}_\ell$. 

These \emph{Circuit Computing} gadgets have two separate functionalities:
the \emph{write mode} ($Control_\ell = 0$) 
and the \emph{compute mode} ($Control_\ell = 1$). When $\text{\emph{C}}_\ell$ is in the \emph{write mode}
the values of the input vertices $\text{\emph{I}}_\ell$ are changed. When $\text{\emph{C}}_\ell$ is in the \emph{compute mode} the values of the vertices $\text{\emph{Next}}\ell$,$\text{\emph{Val}}_\ell$ are updated with the correct output values of the circuit \emph{C}. To formalize the term \emph{correct}, we introduce the following notation that we use through the section.

\begin{definition}\label{d:1}
For the given circuit \emph{C} of \cf{}. We denote with: 
\begin{itemize}
        \item $\text{\emph{Real-Val}}(I_\ell)$ the value of the circuit \emph{C} with input string defined by the values of the vertices in $I_\ell$.
    
    \item $\text{\emph{Real-Next}}(I)_\ell)$ is a 
    neighbor string (Hamming distance \emph{1}) of $I_\ell$ with strictly greater output value in circuit \emph{C}. If such a string does not exist, $\text{\emph{Real-Next}}(I_\ell) = I_\ell$.
\end{itemize}
\end{definition}

The \emph{Comparator} gadget compares $\text{\emph{Val}}_A$ and $\text{\emph{Val}}_B$, which are intended to be $\text{\emph{Real-Val}}(I_A)$, $\text{\emph{Real-Val}}(I_B)$
and outputs \emph{1} if $\text{\emph{Val}}_A \leq \text{\emph{Val}}_B$ or \emph{0} otherwise.
The result of this comparison is ``\emph{stored}'' in the value 
of the \emph{Flag} vertex. If $\text{\emph{Flag}} = 1$ 
then $\text{\emph{I}}_B$ ``\emph{writes}'' her better neighboring solution to $\text{\emph{I}}_A$ (symmetrically if $\text{\emph{Flag}} = 0$).
Intuitively, if this happens 
then 
in the next ``\emph{cycle}'' $\text{\emph{I}}_A$ will have a better value
and will write her improving solution to $\text{\emph{I}}_B$. This goes on and on until no better
neighbor solution exists and both $\text{\emph{I}}_A$ and $\text{\emph{I}}_B$ have the same output vertex values. 

The \emph{CopyB} gadget (respectively for \emph{CopyA}) is responsible for writing the values of the vertices \emph{NextB} to the vertices $\text{\emph{I}}_A$ when
$\text{\emph{Flag}} = 1$ (when $\text{\emph{Val}}_A \leq \text{\emph{Val}}_B$). When $\text{\emph{Flag}} = 1$ the vertices $\text{\emph{T}}_B$ take the values of the vertices in \emph{NextB}. Now if $\text{\emph{I}}_A \neq \text{\emph{NextB}}$ then the $Equality$ gadget turns the value of the \emph{ControlA} to $0$ because $\text{\emph{I}}_A \neq T_B$.
Thus $\text{\emph{C}}_A$  enters \emph{write mode}
and the vertices in $\text{\emph{I}}_A$ adopt the values of the $\text{\emph{Next}}B$ vertices. Then $\text{\emph{Control}}A$ becomes $1$ since $\text{\emph{I}}_A = T_B$ and $\text{\emph{C}}_A$ enters  ``\emph{compute mode}''. This means that
values $\text{\emph{Real-Next}}(I_A)$, $\text{\emph{Real-Val}}(I_A)$ are written to the \emph{output vertices} $\text{\emph{Next}}A$, $\text{\emph{Val}}_A$.

Before proceeding we present a proof-sketch of our reduction. The mathematically rigorous version of this proof is presented in the proof of Theorem~\ref{t:main_max_cut} at the end of the section. We will prove that at any equilibrium of
the instance of \lnmc{} of Figure~\ref{f:construction}
in which $\text{\emph{Flag}} =1$ (symmetrically if $\text{\emph{Flag}} =0$) three things hold:

\begin{enumerate}
    \item $\text{\emph{I}}_A= \text{\emph{Next}}B$
    \item $\text{\emph{Next}}B = \text{\emph{Real-Next}}(I_B)$
    \item $\text{\emph{Real-Val}}(I_B) \geq \text{\emph{Real-Val}}(I_A)$
\end{enumerate}

\noindent Once these claims are established we can be sure that
the string defined by the values of vertices in $I_B$ defines a locally optimal solution for \cf{}. This is because the above $3$ claims directly imply that
$\text{\emph{Real-Val(I}}_B) \geq \text{\emph{Real-Val}} \lp(  \text{\emph{Real-Next}}\lp(I_B\rp)\rp)$ which means that there is no neighboring solution of $I_B$ with strictly greater cost. Obviously we establish symmetrically the above claims when $\text{\emph{Flag}} =0$.  

\begin{remark}\label{rem:0or1??}
Since our construction in Figure~\ref{f:construction} is an instance of \lnmc{} and the bitwise complement of an
equilibrium is also equilibrium the term $\text{\emph{Flag}} = 1$ seems meaningless.
In the construction of the \emph{Circuit Computing} gadget in Section~\ref{s:computing_gadgets} (and in the constructions of all
the presented gadgets) 
there also exist two \emph{supervertices}, a $1$-vertex and a $0$-vertex, with huge weight
that share an edge. As a result, at any equilibrium these vertices have opposite values.
The term $\text{\emph{Flag}} = 1$ means that the \emph{Flag} vertex has the same value with the $1$-vertex.
This notation is also used in subsequent lemmas and always admits the same interpretation. As one can see in the appendix,
the construction of the gadgets assume vertices with values always $0$ or $1$. This can be easily established by connecting one such vertex with its complementary  \emph{supervertex}.
\end{remark}

In the rest of the section we present the necessary lemmas to make the above presented proof sketch rigorous. To do so, we follow a three step approach.  We first present the exact behavior of the \emph{Circuit Computing} gadgets $C_A,C_B$. We then reason why $I_A = \text{\emph{Next}}B$, which we refer to as the \emph{Feedback problem}. Finally we establish the last two claims which we refer to as \emph{Correctness of the Outputs}.

\smallskip
\noindent \textbf{Circuit-computing gadgets}\\
The \emph{Circuit Computing} gadgets $C_A,C_B$ are  
the basic primitives of our reduction
and are based on the gadgets introduced by Sch\"affer and Yannakakis \cite{SY91} to establish
PLS-completeness of \lmc{}. This type of gadgets can be constructed so as to simulate any boolean circuit $C$.
The most important vertices are those corresponding to the input and the output of the
simulated circuit $C$ and are
denoted as $I,O$. The other important vertex is the
\emph{Control} that switches between the \emph{write} and the
\emph{compute mode} of the gadget.
Figure~\ref{f:CGadget} is an abstract depiction of this type of gadgets.
The properties of the gadget are described in Theorem~\ref{l:SY_gadgets}. Its proof is presented in
Section~\ref{s:computing_gadgets}, where the exact construction of the gadget is presented.
We first introduce some convenient notation that will help us
throughout the proof of completeness.

\begin{figure}[h]
    \centering
    \includegraphics[scale =0.7]{CGadget.jpg}
    \caption{\emph{Circuit Computing} gadgets. The big, dashed ``vertices'' named I and O, represent all the input and output vertices respectively. This type of (``hyper''-)vertex is represented in the rest of the figures with a bold border.}
\label{f:CGadget}
\end{figure}

\begin{definition}\label{d:bias}
Let an instance of \lnmc{} and a specific equilibrium of this instance. The \emph{bias} that vertex $i$ experiences with respect to the subset $N' \subseteq N$ is
\[\lp|\sum_{j \in N_i^1  \cap N'}w_j -\sum_{j \in N_i^0 \cap N' }w_j \rp|\]
where $N_i^0$ is the set of neighbors of vertex $i$ that choose $0$ (respectively for $N_i^1$)
\end{definition}

Bias is a key notion in the subsequent analysis. The gadgets presented in Figure~\ref{f:construction}
are a subset of the vertices of the overall instance. Each gadget is composed by the "input vertices", the internal vertices and the "output vertices". Moreover as we have seen
each gadget stands for a "circuit" with some specific functionality (computing, comparing, copying e.t.c.). Each gadget is specifically constructed so as at any equilibrium of the overall instance, the output vertices of the gadget experience some bias towards some values that depend on the values of the input vertices of the gadget. 
Since the output vertices of a gadget may also participate as input vertices at some other gadgets, it is important to quantify the bias of each gadget in order to prove consistency in our instance. Ideally, we would like to prove that at any equilibrium the bias that a vertex experiences from a gadget in which it is an output vertex, is greater than the sum of the biases of the gadgets in which it participates as input vertex.

Theorem~\ref{l:SY_gadgets}
describes the equilibrium behavior of the input vertices $I_\ell$ and output vertices $Next\ell,Val_\ell$ of the $Circuit Computing$ gadgets $C_\ell$.

% cp
\begin{restatable}{theorem}{sygadgets}
\label{l:SY_gadgets}
\noindent
At any equilibrium of the \lnmc{} of Figure~\ref{f:construction}. 

\begin{enumerate}
    \item If $Control\ell = 1$ and the vertices of $Next\ell$,$Val_\ell$ experience $0$ bias from any other gadget beyond $C_\ell$ then:
    
    \begin{itemize}
        \item $\text{\emph{Next}}\ell = \text{\emph{Real-Next}}(I_\ell)$
    
        \item $\text{\emph{Val}}_\ell = \text{\emph{Real-Val}}(I_\ell)$
    
     \end{itemize}
    
    \item If  $Control\ell = 0$ then 
    each vertex in $I_\ell$ experiences $0$
    bias from the internal vertices of $C_\ell$.
    
    \item $Control\ell$ experiences
    $w_{Control\ell}$ bias from the internal vertices of $C_\ell$.
\end{enumerate}
\end{restatable}
%\end{replemma}

\noindent Case~$1$ of Theorem~\ref{l:SY_gadgets}
describes the \emph{compute mode} of the \emph{Circuit Computing} gadgets. 
At any equilibrium with $ControlA =1$, and with the output vertices of $C_A$ being indifferent with respect to other gadgets, then $C_A$ computes its output correctly. Note that because the vertices in \emph{NextA},\emph{ValA} are also connected with internal vertices of other gadgets
(\emph{CopyA} and \emph{Comparator} gadgets)
that may create bias towards the opposite value, the second condition is indispensable. Case~$2$ of Theorem~\ref{l:SY_gadgets} describes the \emph{write mode}. If at an equilibrium $ControlA = 0$ then the vertices in $I_A$ have $0$ bias from the $C_A$ gadget and as a result their value is determined by the biases of the \emph{CopyB} gadget and the \emph{Equality} gadget. Case~$3$ of Theorem~\ref{l:SY_gadgets} describes the minimum bias that the equality gadget must pose to the Control vertices 
so as to make the computing gadget flip from one mode to the other. As we shall see, the weights $w_{ControlA} = w_{ControlB} = w_{Control}$ are selected much smaller than the bias the $Control\ell$ vertices experience due to 
the \emph{Equality} gadgets, meaning that the \emph{Equality} gadgets control the \emph{write mode} and the \emph{compute mode} of the \emph{Circuit Computing} gadgets no matter the values of the vertices in $C_\ell$ gadgets.
\begin{remark}\label{r:5}
We remark that our construction of the \emph{Circuit Computing} gadgets presented in Section~\ref{s:computing_gadgets} ensures Theorem~\ref{l:SY_gadgets} for selecting $w_{Control}$ arbitrarily smaller than the
weights for the internal vertices of the \emph{Circuit Computing} gadgets. As we shall see up next this is crucial for our reduction and, as we discuss in the end of the section, this is a major difference with the respective \emph{Circuit Computing} gadgets of other reductions in this vein \cite{SY91,GS10,ET11}.
\end{remark}

\smallskip
\noindent \textbf{Solving the Feedback problem.}\\
The purpose of this section is to establish the first case of the above presented claims i.e. at any equilibrium of \lnmc{}
instance of Figure~\ref{f:construction}
in which $\text{\emph{Flag}} = 1$,
\emph{NextB} is written to $I_A$ and vice versa when $\text{\emph{Flag}} = 0$. This is formally stated in Theorem~\ref{l:write}.


\begin{theorem}
\label{l:write}
Let an equilibrium of the instance of \lnmc{}
described in Figure~\ref{f:construction}.
\begin{itemize}
    \item If $\text{\emph{Flag}} = 1$ then $I_A = \text{\emph{NextB}}$
    \item If $\text{\emph{Flag}} = 0$ then $I_B = \text{\emph{NextA}}$
\end{itemize}
\end{theorem}


\noindent We next present the necessary lemmas for proving Theorem~\ref{l:write}.

\begin{restatable}{lemma}{consistent}
\label{l:consistent1}

Let an equilibrium of the overall \lnmc{} instance of Figure~\ref{f:construction}. Then 
\begin{itemize}
    \item $ControlA = (I_A  =  T_B)$
    \item $ControlB = (I_B  =  T_A)$
\end{itemize}
\end{restatable}
%\end{replemma}

\noindent In Section~\ref{s:control} we present the construction of the equality gadget. This gadget is specifically designed so that at any equilibrium, its internal vertices create bias to 
$ControlA$ towards the value of the predicate $(I_A  =  T_B)$.
Notice that if we multiply
all the internal vertices of the equality gadget with a positive constant, the bias $ControlA$ experiences
towards value $(I_A  =  T_B)$ is multiplied by the same constant (see Definition~\ref{d:bias}). Lemma~\ref{l:consistent1} is established
by multiplying these weights
with a  sufficiently large
constant so as to make this bias larger than $w_{ControlA}$.
We remind that by Theorem~\ref{l:SY_gadgets}, the bias that $ControlA$ experiences from $C_A$ is $w_{ControlA}$. As a result, the equilibrium value of $ControlA$ is $(I_A  =  NextB)$ no matter the values of $ControlA$ 's neighbors in the $C_1$ gadget.
The \emph{red mark} between $ControlA$ and the $C_A$ gadget in Figure~\ref{f:construction} denotes the "indifference" of $ControlA$ towards the values of the $C_A$ gadget (respectively for $ControlB$).

In the high level description of the 
\lnmc{} instance of Figure~\ref{f:construction}, when $\text{\emph{Flag}} = 1$
the values of \emph{NextB} is copied to $I_A$ as follows: At first $T_B$ takes the value of \emph{NextB}. If $I_A \neq T_B$ then $ControlA = 0$
and the $C_A$ gadget switches to \emph{write mode}. Then the vertices in $I_A$ takes the values of the vertices in \emph{NextB}. This is formally stated in Lemma~\ref{l:copy2}.

%\begin{replemma}{l:copy2}
\begin{restatable}{lemma}{copyB}
\label{l:copy2}
At any equilibrium point of the \lnmc{} instance of Figure~\ref{f:construction}:
\begin{itemize}
    \item If $\text{\emph{Flag}} = 1$, i.e. \emph{NextB} \emph{writes} on $I_A$, then 
    
        \begin{enumerate}
                \item $T_B = \text{\emph{NextB}}$
        
                \item If $ControlA = 0$ then $I_A = T_B = \text{\emph{NextB}}$
        \end{enumerate}

\item If $\text{\emph{Flag}} = 0$ i.e. \emph{NextA} \emph{writes} on $I_B$, then 
    
        \begin{enumerate}
                \item $T_A = \text{\emph{NextA}}$
        
                \item If $ControlB = 0$ then $I_B = T_A = \text{\emph{NextA}}$
        \end{enumerate}
\end{itemize}
\end{restatable}
%\end{replemma}

\noindent In Section~\ref{s:copy}, we present the construction of the \emph{Copy} gadgets. At an equilibrium where $\text{\emph{Flag}} = 1$, this gadget creates bias to the vertices in $I_A,T_B$ vertices towards adopting the values of \emph{NextB}. Since $I_A,T_B$
also participate in the \emph{Equality} gadget in order to establish Lemma~\ref{l:copy2} we want to make the bias of the \emph{CopyB} gadget larger than the bias of the \emph{Equality} gadget. This is done by again by multiplying the weights of the internal vertices of \emph{CopyB} with a sufficiently large constant. The "indifference" of the vertices in $I_A,T_B$ with respect to the values of the internal vertices of the \emph{Equality} gadget is denoted
in Figure~\ref{f:construction}
by the \emph{red marks} between the vertices in $I_A,T_B$ and the \emph{Equality} gadget.


In Case~$2$ of Lemma~\ref{l:copy2} the additional condition $ControlA = 0$ is necessary to ensure that $I_A = \text{\emph{NextB}}$. The reason is that the bias of the \emph{Copy} gadget to the vertices in $I_A$ is sufficiently larger than the bias of the \emph{Equality} gadget to the vertices in $I_A$, but not necessarily to the bias of the $C_A$ gadget. The condition $ControlA = 0 $ ensures $0$ bias of the $C_A$ gadget to the vertices $I_A$, by Theorem~\ref{l:SY_gadgets}. As a result the values of the vertices in $I_A$ are determined by the values of their neighbors in the \emph{CopyB} gadget.


\begin{proof}[Proof of Theorem~\ref{l:write}]
Let an equilibrium in which $\text{\emph{Flag}} = 1$.
Let us assume that $I_A \neq \text{\emph{NextB}}$.
By Case~$1$ of Lemma~\ref{l:copy2}, $T_B = \text{\emph{NextB}}$. As a result, $I_A \neq T_B$, implying that $ControlA = 0$ (Lemma~\ref{l:consistent1}). Now, by Case~$2$ of Lemma~\ref{l:copy2} we have that $I_A = \text{\emph{NextB}}$, which is a contradiction. The exact same analysis holds when $\text{\emph{Flag}} = 0$.
\end{proof}

\smallskip
\noindent \textbf{Correctness of the Output Vertices.}

\noindent In the previous section we discussed how the \emph{Feedback problem} ($I_A = \text{\emph{NextB}}$ when $\text{\emph{Flag}} = 1$) is solved in our reduction.
We now exhibit how the two last cases of our initial claim are established.
\begin{theorem}\label{t:2}
At any equilibrium of the instance of \lnmc{} of
Figure~\ref{f:construction}:
\begin{itemize} 
\item If $\text{\emph{Flag}} = 1$
    \begin{enumerate}
    \item $\text{\emph{Real-Val}}(I_A) \leq \text{\emph{Real-Val}}(I_B)$
    \item $\text{\emph{NextB}} = \text{\emph{Real-Next}}(I_B)$
\end{enumerate}

\item If $\text{\emph{Flag}} = 0$
    \begin{enumerate}
    \item $\text{\emph{Real-Val}}(I_B) \leq \text{\emph{Real-Val}}(I_A)$
    \item $\text{\emph{NextA}} = \text{\emph{Real-Next}}(I_A)$
\end{enumerate}
\end{itemize}
\end{theorem}

At first we briefly explain the difficulties in establishing Theorem~\ref{t:2}. In the following discussion we assume that $\text{\emph{Flag}} = 1$, since everything we mention holds symmetrically for $\text{\emph{Flag}} = 0$. Observe
that if $\text{\emph{Flag}} = 1$ we know nothing about the value of $ControlB$ and as a result we cannot guarantee that
$\text{\emph{NextB}}  = \text{\emph{Real-Next}} (I_B)$ or $\text{\emph{Val}}_B = \text{\emph{Real-Val}}(I_B)$. But even in the case of $C_A$ where $ControlA = 1$ due to Theorem~\ref{l:write},
the correctness of the vertices in $\text{\emph{NextA}}$ or $\text{\emph{Val}}_A$ cannot be guaranteed.
The reason is that in order to apply Theorem~\ref{l:SY_gadgets}, \emph{NextA} and $\text{\emph{Val}}_A$ should experience $0$ bias with respect to
any other gadget they are connected to. But at an equilibrium, these vertices may select their values according to the values of their \emph{heavily weighted neighbors} in the \emph{CopyA} and the \emph{Comparator} gadget.

The correctness of the values of the output vertices, i.e. $\text{\emph{NextA}} = \text{\emph{Real-Next}}(I_A)$ and $\text{\emph{Val}}_A = \text{\emph{Real-Val}}(I_A)$, is ensured
by the design of the \emph{CopyA} and the \emph{Comparator} gadgets. Apart from their primary role these gadgets are specifically designed to
cause $0$ bias to the output vertices of the \emph{Circuit Computing} gadget to which
the better neighbor solution is written. In other words at any equilibrium in which $\text{\emph{Flag}} = 1$ and any vertex in $C_A$:
the total weight of its neighbors (belonging in the \emph{CopyA} or the \emph{Comparator} gadget) with value $1$
equals the total weight of its neighbors (belonging in the \emph{CopyA} or the \emph{Comparator} gadget) with value $0$.

The latter fact is denoted by the \emph{green marks} in Figure~\ref{f:construction_1} and permits the application of Case~$1$ of Theorem~\ref{l:SY_gadgets}.
Lemma~\ref{l:copy_unbias} and ~\ref{l:comparator_unbias} formally state these "green marks".

\begin{figure}
    \centering
    \includegraphics[scale= 0.5]{ArchFlag1.jpg}
    \caption{Since $Flag = 1$ any internal vertex of the $C_2$ gadget has $0$ bias with respect to all the other gadgets. As a result, Theorem~\ref{l:SY_gadgets} applies.}
\label{f:construction_1}
\end{figure}


%\begin{replemma}{l:copy_unbias}
\begin{restatable}{lemma}{copyUnbias}
\label{l:copy_unbias}
At any equilibrium point of the \lnmc{} instance of Figure~\ref{f:construction}:
\begin{itemize}
    \item If $\text{\emph{Flag}} = 1$ then any vertex in \emph{NextA} experience $0$ bias with respect to the \emph{CopyA} gadget.
        

\item If $\text{\emph{Flag}} = 0$ then 
then any vertex in \emph{NextB} experience $0$ bias with respect to the \emph{CopyB} gadget.
\end{itemize}
\end{restatable}
%\end{replemma}
\newpage
%\begin{replemma}{l:comparator_unbias}
\begin{restatable}{lemma}{comparatorUnbias}
\label{l:comparator_unbias}
Let an equilibrium of the instance of \lnmc{} of Figure~\ref{f:construction}:

\begin{itemize}
    \item If \emph{Flag} = 1 then all vertices of $C_A$ experience $0$ bias to the \emph{Comparator} gadget.
    
    \item If \emph{Flag} = 0 then all vertices of $C_B$ experience $0$ bias to the \emph{Comparator} gadget.
\end{itemize}
\end{restatable}
%\end{replemma}

\begin{remark}
The reason that in Lemma~\ref{l:comparator_unbias} we refer to all vertices of $C_A$ (respectively $C_B$) and not just to the vertices in $Val_A$ (respectively $Val_B$) is that in the constructed instance of \lnmc{} of Figure~\ref{f:construction}, we connect internal vertices of the $C_A$ gadget with internal vertices of the \emph{Comparator} gadget. This is the only point in our construction where internal vertices of different gadgets share an edge and is denoted in Figure~\ref{f:construction} and~\ref{f:construction_1} with the direct edge between the $C_A$ gadget and the \emph{Comparator} gadget.
\end{remark}

\noindent Now using Lemma~\ref{l:copy_unbias} and Lemma~\ref{l:comparator_unbias} we can prove the correctness of the output vertices $\text{\emph{NextA}}, \text{\emph{Val}}_A$ when $\text{\emph{Flag}} =1$ i.e. 
$\text{\emph{NextA}} = \text{\emph{Real-Next}}(I_A)$ and $\text{\emph{Val}}_A = \text{\emph{Real-Val}}(I_B)$ (symmetrically
for the vertices in
$\text{\emph{NextB}}, \text{\emph{Val}}_B$ when
$\text{\emph{Flag}} = 0$).

%\begin{replemma}{l:correctness1}
\begin{restatable}{lemma}{correctnessA}
\label{l:correctness1}
Let an equilibrium of the instance of \lnmc{} of Figure~\ref{f:construction}:
\begin{itemize}
    \item If $\text{\emph{Flag}} = 1$ then $\text{\emph{NextA}} = \text{\emph{Real-Next}}(I_A)$, $\text{\emph{Val}}_A =  \text{\emph{Real-Val}}(I_A)$.
    \item If $\text{\emph{Flag}} = 0$ then $\text{\emph{NextB}} = \text{\emph{Real-Next}}(I_B)$, $\text{\emph{Val}}_B =  \text{\emph{Real-Val}}(I_B)$.
\end{itemize}
\end{restatable}
%\end{replemma}

\begin{proof}
We assume that $\text{\emph{Flag}} = 1$ (for $\text{\emph{Flag}} = 0$ the exact same arguments hold). By Theorem~\ref{l:write} we have $I_A = \text{\emph{NextB}}$ and by Lemma~\ref{l:copy2} we have that $T_B = \text{\emph{NextB}}$. As a result, $I_A = T_B$ and by Lemma~\ref{l:consistent1}
$ControlA = 1$.
Lemma~\ref{l:copy_unbias} and Lemma~\ref{l:comparator_unbias} guarantee that the vertices in $\text{\emph{NextA}},\text{\emph{Val}}_A$ of $C_A$ experience $0$ bias towards all the other gadgets of the construction and since $ControlA = 1$,
we can apply Case~$1$ of Theorem~\ref{l:SY_gadgets} i.e. 
$\text{\emph{Val}}_A = \text{\emph{Real-Val}}(I_A)$ and 
$\text{\emph{NextA}}= \text{\emph{Real-Next}}(I_A)$.
\end{proof}

Up next we deal with the correctness of the values of the output vertices in $\text{\emph{Val}}_B$ and $\text{\emph{NextB}}$ when $\text{\emph{Flag}} = 1$.
We remind again that, even if at an equilibrium $ControlB=1$, we could not be sure about the correctness
of the values of these output vertices due to the bias their neighbors in the \emph{CopyB} and the \emph{Comparator} gadget (Theorem~\ref{l:SY_gadgets} does not apply).
The \emph{Comparator} gadget plays a crucial role in solving this last problem.
Namely, it also checks whether the output vertices in \emph{NextB} have correct values with respect to the input $I_B$ and
if it detects incorrectness it outputs $0$. This is done by
the connection of some specific internal vertices
of the $C_A,C_B$ gadgets with the internal vertices of the \emph{Comparator} gadget (Figure~\ref{f:construction}: edges between $C_A,C_B$ and \emph{Comparator}).

%\begin{replemma}{l:comparator_correctness}
\begin{restatable}{lemma}{comparatorCorrectness}
\label{l:comparator_correctness}
At any equilibrium of the \nmc{} instance of Figure~\ref{f:construction}: 

\begin{itemize}
    \item If $\text{\emph{Flag}} = 1$ then $\text{\emph{NextB}} = \text{\emph{Real-Next}}(I_B)$
    
    \item If $\text{\emph{Flag}} = 0$
     then $\text{\emph{NextA}} = \text{\emph{Real-Next}}(I_A)$
\end{itemize}
\end{restatable}
%\end{replemma}

\noindent We highlight that the correctness of values of the output vertices \emph{NextB}, i.e. $\text{\emph{NextB}} = \text{\emph{Real-Next}}(I_B)$, is not guaranteed by application of Theorem~\ref{l:SY_gadgets} (as in the case of correctness of $NextA,Val_A$), but from the construction of the \emph{Comparator} gadget. Lemma~\ref{l:comparator_correctness} is proven in Section~\ref{s:comparison_gadget} where the exact construction of this gadget is presented. Notice that Lemma~\ref{l:comparator_correctness} says nothing about the correctness of the values of the output vertices in $Val_B$. As we latter explain this cannot be guaranteed in our construction. Surprisingly enough, the \emph{Comparator}
outputs the right outcome of the predicate $\lp(\text{\emph{Real-Val}}(I_A) \leq \text{\emph{Real-Val}}(I_B)\rp)$ even if
$\text{\emph{Val}}_B \neq \text{\emph{Real-Val}}(I_B)$. The latter is one of our main technical contributions in the reduction that reveals the difficulty of \lnmc{}. The crucial differences between our \emph{Comparator} and the \emph{Comparator} of the previous reductions \cite{SY91,GS10,ET11} are discussed in the end of the section. Lemma~\ref{l:comparator} formally states the robustness of the outcome of the \emph{Comparator} even with "wrong values"
in the vertices of $Val_B$ and is proven in Section~\ref{s:comparison_gadget}.


% cp
%\begin{replemma}{l:comparator}
\begin{restatable}{lemma}{comparator}
\label{l:comparator}
At any equilibrium of the \lnmc{} instance of Figure~\ref{f:construction}:

\begin{itemize}
    \item If $Flag = 1$, $\text{\emph{NextA}} = \text{\emph{Real-Next}}(I_A)$,
    $\text{\emph{Val}}_A = \text{\emph{Real-Val}}(I_A)$
    and $\text{\emph{NextB}} = \text{\emph{Real-Next}}(I_B)$
    then
    \[Real-Val(I_A) \leq Real-Val(I_B)\]
    
    \item If $Flag = 0$, $\text{\emph{NextB}} = \text{\emph{Real-Next}}(I_B)$,
    $\text{\emph{Val}}_B = \text{\emph{Real-Val}}(I_B)$
    and $\text{\emph{NextA}} = \text{\emph{Real-Next}}(I_A)$
    then
    \[Real-Val(I_B) \leq Real-Val(I_A)\]
\end{itemize}
\end{restatable}
%\end{replemma}
\noindent We are now ready to prove Theorem~\ref{t:2}.

%simantiki apodeiksi
\begin{proof}[Proof of Theorem~\ref{t:2}]

Let an equilibrium of the instance of Figure~\ref{f:construction} with $\text{\emph{Flag}} = 1$ (respectively for $\text{\emph{Flag}} = 0$).
By Lemma~\ref{l:comparator_correctness}, $\text{\emph{NextB}} = \text{\emph{Real-Next}}(I_B)$ and thus Case~$1$ is established. 
Moreover by Lemma~\ref{l:correctness1}, $\text{\emph{NextA}} = \text{\emph{Real-Next}}(I_A)$ and $\text{\emph{Val}}_A = \text{\emph{Real-Val}}(I_A)$. As a result,
Lemma~\ref{l:comparator} applies and $\text{\emph{Real-Val}}(I_A) \leq \text{\emph{Real-Val}}(I_B)$ (Case~$2$ of Theorem~\ref{t:2})
\end{proof}

\noindent Having established Theorem~\ref{l:write} and \ref{t:2} the $PLS$-completeness of \lnmc{}
follows easily. For the sake of completeness we present the proof of Theorem~\ref{t:main_max_cut} that we describe in the beginning of the section. 

\begin{theorem}\label{t:main_max_cut}
\lnmc{} is PLS-complete.
\end{theorem}
\begin{proof}
For a given circuit $C$ of the \cf{}, we can construct in polynomial time the instance of \lnmc{} of Figure~\ref{f:construction}. 
Let an equilibrium of this instance. Without loss of generality, we assume that $Flag = 1$.
Then, by Theorem~\ref{l:write} and Theorem~\ref{t:2}, $I_A = NextB$, $NextB = Real-Next(I_B)$ and $Real-Val(I_A) \leq Real-Val(I_B)$. As a result, we have that 
\begin{eqnarray*}
Real-Val(I_B) &\geq& Real-Val(I_A)\\
&=& Real-Val(NextB)\\
&=& Real-Val\lp( Real-Next(I_B) \rp)
\end{eqnarray*}
But if $I_B \neq Real-Next(I_B)$, by Definition~\ref{d:1} then $Real-Val(I_B)  > Real-Val\lp( Real-Next(I_B) \rp)$ which is a contradiction.
Thus $I_B = Real-Next(I_B) = I_B$, meaning that the string defined by the values of $I_B$ is a locally optimal solution for the \cf{} problem.  
\end{proof}

\smallskip
\noindent \textbf{Our technical contributions}

As already mentioned the construction of Figure~\ref{f:construction} follows the \emph{flip-flop architectures} of previous PLS reductions ~\cite{SY91,GS10,ET11}.
In all these reduction the selection of the weights in the connecting edges played a crucial role. We briefly discuss the points of our reduction,
which are at the heart of the PLS-completeness proof of \lnmc{}.

Our \emph{Circuit Computing} gadgets are based on the
\emph{Circuit Computing} gadgets introduced by Sch\"affer and Yannakakis \cite{SY91} (and used by Els\"asser et al for similar problems \cite{GS10,ET11}).
There is one major modification of these gadgets, which
concerns Case~$3$ of Theorem~\ref{l:SY_gadgets}. Our \emph{Circuit Computing} gadgets can be constructed
with the weight $w_{Control}$ being arbitrarily smaller than the weights of the
other vertices of the \emph{Circuit Computing} gadget.
The importance of this property for our reduction is twofold: 
At first, Case~$3$ guarantees the $Control$ vertex will have very small \emph{bias} with respect to the \emph{Circuit Computing} gadget.
This is very important since we were able to select the weights in the \emph{Equality} gadget
large enough so as to control the \emph{write} and the \emph{compute} mode
but at the same time small enough so as not to affect the values of "\emph{input vertices}" $I_A,I_B$.  
The second crucial
reason that necessitates $w_{Control}$ being small is that $Control$ should follow the "\emph{output}"
of the \emph{Equality} gadget and not vice versa.
It is here that the main difference between the \lnmc{} problem and the original \lmc{} arises.
The major difference between the \emph{Circuit Computing} gadgets introduced by Sch\"affer and Yannakakis  \cite{SY91}
and ours, is that the $Control$ vertex has small bias with respect to the \emph{Circuit Computing} gadget but weight comparable to the weights of the internal vertices
of the \emph{Circuit Computing} gadget. All these reductions ensure that $Control$ does not influence
its neighbors (outside the circuit computing gadget) by selecting sufficiently small weights in the
edges, something that cannot be done in the \lnmc{} problem.
Our first main technical contribution is establishing Cases~$1$ and~$2$ with the $Control$ vertex
having arbitrarily smaller weight than the other vertices in the gadget.
To achieve so we design a \emph{Leverage} gadget that is internally used in the
\emph{Circuit Computing} gadget.
This gadget reduces the influence of a vertex with large weight to a vertex with small weight and is presented in Section~\ref{s:leverage}.

The second important difference of our reduction concerns the \emph{red marks}
between the \emph{Flag}
and the \emph{Copy} gadgets in Figure~\ref{f:construction}. These
\emph{red marks} indicate
that \emph{Flag} vertex takes the output of the \emph{Comparator} gadget. These marks are more tricky to establish than the other \emph{red marks} in Figure~\ref{f:construction}. The reason is that both the \emph{Comparator} and the \emph{Copy} gadgets have input vertices in $NextA, NextB, Val_A, Val_B$ which have weights of the same order of magnitude as output vertices of the \emph{Circuit Computing} gadgets. As a result, this time the weights of the internal vertices in the \emph{Comparison} gadget cannot be selected sufficiently larger than the respective weights of the \emph{Copy} gadgets. In the work of Sch\"affer and Yannakakis \cite{SY91,GS10,ET11}
the bias of the \emph{Flag} from the \emph{Copy} gadgets was made negligible to the respective bias from
the \emph{Comparator} by connecting the \emph{Flag} with the \emph{Copy} gadgets with edges of sufficiently small weight.
This is the second point where the absence of weights on the edges plays a major role. We overcome this difficulty by again using the \emph{Leverage} gadget internally in the \emph{Copy} gadget. Now the  \emph{Leverage} gadget
decreases the influences of the internal vertices of the \emph{Copy} gadgets to the
\emph{Flag} making its bias much smaller than the bias of the \emph{Comparator}. This is formally established in Lemma~\ref{l:comparator}.

Our final major technical contribution concerns the design of the \emph{Comparator} gadget. As stated in Lemma~\ref{l:comparator}
our \emph{Comparator} outputs $\lp ( \text{\emph{Real-Val}}(I_A) \geq \text{\emph{Real-Val}}(I_A) \rp )$ even if some "\emph{input~vertices}" of the \emph{Comparator} have incorrect values. In the previous reductions the \emph{Comparator} guaranteed correctness both on the values of the vertices in $\text{\emph{Next}}B$, $\text{\emph{Val}}_B$
by the use of the suitable weights on the connecting edges. Having the correct "input values", the comparison step is quite straightfoward to implement. This decoupled architecture of the \emph{Comparator} could not be implemented with a \lnmc{} instance, due to the absence of edge-weights, and we had to deploy an \emph{all at once} \emph{Comparator} that ensures correctness to some of its input vertices so as to perform correctly the comparison step.


==> nodeMaxCut.tex <==
\section{Node Max-Cut}\label{sec:nodeMaxCut}
\subsection{Main (Stratis)}

In this section we present the proof of Theorem~\ref{t:main_max_cut}
which states that \nmc{} is \emph{PLS}-complete.
We reduce an instance of  \cf{} to
an instance of  \nmc{}. 
%In the \cf{} we are given a circuit $C$ with $n$ input gates and $m$ output gates. The value of $n$-bit input string $I$ is the $m$-bit integer in the output gates. Given such a circuit $C$, we need to find a input string $I$ such as if we flip the value of any bit of $I$ the value of the produced string does not increase.


\thl{Initially, reducing \cf{} to \nmc{} might seem fairly simple by observing that} %The main reason that \cf{} can be reduced to \nmc{} is fairly simple 
any circuit $C$ can be represented as a DAG of \emph{NOR}-gates with fan-in $2$ and each \emph{NOR}-gate can be simulated by a simple instance of  \nmc{}  \thl{on five nodes} (Figure~\ref{f:Node_Nor}). By selecting the weights %$x$
\thl{of these five nodes} in each \emph{NOR}-gadget in an exponentially decreasing \thl{manner} from left to right we can ensure the consistency of the gadget, i.e., %More precisely, 
at any equilibrium of the  constructed \nmc{} instance the values of the \emph{input} nodes $I$ and the values of the output nodes \emph{O} satisfy $O = C(I)$.

\begin{figure}
    \centering
    \includegraphics[scale=1]{figures/NodeNor.jpg}
    \caption{A gadget simulating a NOR gate. The label of each node defines its weight. The common variable $x$ appearing in all nodes can be any number (this freedom is very helpful in our gadgets). The square node is fixed to always play  value $1$ by connecting it to a very heavy node  outside the gadget. Each input node connects to an external node with weight greater than $x$. This way, independent of what the middle $x$ node plays, each of the $2x$ nodes plays the opposite value than the value that their corresponding external node played.}
\label{f:Node_Nor}
\end{figure}

%One might initially consider the following approach. 
Given a circuit $C$, \thl{in a fist try, one} can construct in polynomial time a circuit $C_{\overline{Next}}$ that for a given input string $I$,
returns the complement of a neighboring string of $I$ (their Hamming distance is $1$) with strictly greater cost. If such a neighbor string does not exist $C_{\overline{Next}}$ outputs the complement of $I$. Now consider an instance of \nmc{} simulating the circuit $C_{\overline{Next}}$ in the way that we described above and with additional edges between each input node in $I$ and its respective output node in $O$ (Figure \ref{}).
Intuitively at an equilibrium
of this \nmc{} instance the output nodes are the complement of the input nodes, meaning for this input string
circuit $C_{\overline{Next}}$ outputs the negation of the string. As a result, the input string
defined by the values
of the nodes in $I$ has no neighbor string with strictly
greater value and thus is a solution for \cf{} problem.

The problem with the above presented approach is that the weights of the
nodes corresponding to the input $I$ are exponentially greater than the weights
of the other neighbors of nodes in \emph{O}, meaning that a nodes in $O$
will always play the negation of their respective neighbors in $I$ no
matter the values of their neighbors in the rest of the gadget and
thus $O \neq C_{\overline{next}}(I)$.
To solve this fundamental \emph{Feedback Problem} we
we design a more refined circuit-computing gadget that is presented in
Section~\ref{s:computing_gadgets}.
These circuit-computing gadgets (Figure~\ref{f:CGadget}) are the basic primitive of our reduction
and are based on the gadgets presented in \cite{SY91} to establish
PLS-completeness of  \lmc{}. The most important nodes
of this gadget are the nodes corresponding to the input and the output of the
simulated circuit and are
denoted as $I,O$. There is also an additional important node called
$Control$ whose use will be clarified below.
Figure~\ref{f:CGadget} illustrates an abstract description of this type of gadgets.
The exact construction of the circuit-computing
gadgets is presented in Section~\ref{s:computing_gadgets} and its properties
are stated in Lemma~\ref{l:SY_gadgets}.

\begin{figure}
    \centering
    \includegraphics[scale =1]{figures/CGadget.jpg}
    \caption{Circuit-Computing gadgets.}
\label{f:CGadget}
\end{figure}

%\begin{replemma}{l:SY_gadgets}
%HERE!!!
\begin{restatable}{lemma}{SYgadgets}
\label{l:SY_gadgets}
For a given circuit $C$ consider the instance of \nmc{} of Section~\ref{s:computing_gadgets}.
At any equilibrium of this instance:

\begin{enumerate}
    \item If $\emph{Control } = 1$ then $O = C(I)$. Each node in $O$ has bias $\epsilon  < w_{Control}$ towards her equilibrium value.
    
    \item If  $\emph{Control } = 0$ then 
    each node in $I$ has $0$
    bias towards her equilibrium value.
    
    \item The \emph{Control} node has bias
    $w_{Control}$ towards her equilibrium value.
    
\end{enumerate}
\end{restatable}


%\end{replemma}

\begin{remark}\label{r:remark2}
The term bias used in Lemma~\ref{l:SY_gadgets} also appears in the subsequent Lemmas and analysis and it is important to clarify its meaning. Consider an equilibrium of an instance of \nmc{}. Since nodes are at equilibrium, for an agent with equilibrium
value $0$, the total weight of its neighbors with value $1$
is greater than the total weight of the neighbors with value $0$. The bias of this specific agent
is the absolute difference on the total weight of its $1$-neighbors and its $0$-neighbors (see Figure~\ref{}[Bias] for an example).
The reason that notion of bias is convenient is because in our final construction some nodes
participate in several gadgets (each gadget is an instance of
the \nmc{}). If for a given node the bias of one gadget is greater than the sum of the biases of the remaining gadgets
then this node follows the equilibrium value of gadget with the high bias.
\end{remark}

\begin{remark}\label{r:remark}
\begin{itemize}
    \item Circuit-computing gadgets can be implemented with the weight of the Control
node arbitrarily smaller than the weights of the input and output gates.
The only restriction is that the parameter $\epsilon$ which is the weight
of certain internal nodes must be selected sufficiently smaller than $w_{Control}$. Due to the construction of the circuit-computing gadgets, 
$\epsilon$ is the bias of the output agents
towards their equilibrium value
which is the output of the simulated circuit.
\textcolor{red}{supernodes description also found in appendix}
\item Since the gadget is an instance of \nmc{} and the bitwise complement of an
equilibrium is also equilibrium the term $Control = 1$ seems meaningless.
In the construction of the circuit-computing gadget in Section~\ref{s:computing_gadgets} (and in the constructions all of
the presented gadgets) there exists an $1$-node and an $0$-node with huge weight
that share an edge and as a result at any equilibrium these nodes have opposite values.
The term $Control = 1$ means that the $Control$ node has the same value with the $1$-node.
This notation is also used in  subsequent Lemmas and always admits the same interpretation.

\end{itemize}
\end{remark}

Before proceeding we present how these circuit-computing gadgets are used to solve the
\emph{Feedback problem}. Let an equilibrium with $Control = 0$ (Case~$2$),
the input nodes in $I$ experience $0$ bias from their neighbors in the circuit-computing
gadget. Intuitively this means that we can transfer values to the nodes in $I$ from nodes
with weight much smaller than the weight of
internal nodes of the circuit-computing gadget.
On the other hand if $Control = 1$ (Case~$1$) then the values of the
nodes in $O$ will be the output of the simulated circuit $C$. This switching between
the \emph{write mode} and the \emph{compute mode} is the cornerstone for solving the
Feedback problem and has been extensively used in many PLS-completeness reductions
for variants of the original \lmc{} problem \cite{GS10,ET11}.

We now exhibit the importance of Case~$3$ of Lemma~\ref{l:SY_gadgets}. As we shall later see the
weight $w_{Control}$ (see also Section~\ref{s:computing_gadgets}) is selected much smaller than the
weights of the internal nodes of the circuit-computing gadget. The reason for this is twofold.
At first by Case~$3$, the $Control$ node will have very small \emph{bias} with respect to the circuit-computing gadget.
This is very important since we can switch between the \emph{write} and the \emph{compute} mode by
connecting $Control$ with nodes having weight slightly greater than $w_{Control}$. The second crucial
reason that $w_{Control}$ must be small is that $Control$ should be influenced by its neighbors (outside the circuit computing gadget) and not vice versa. It is here that the main differentiation between the \nmc{} problem and the original \lmc{} arises.
The major difference between the circuit-computing gadgets introduced in \cite{SY91} (also used in \cite{GS10},\cite{ET11})
and ours, is that the $Control$ node has small bias with respect to the circuit-computing gadget but weight comparable to the weights of the internal nodes
of the circuit-computing gadget. All these reductions ensure that $Control$ does not influence
its neighbors (outside the circuit computing gadget) by selecting sufficiently small weights in the
edges, something that cannot be done in the \nmc{} problem.
Our first main technical contribution is establishing Case~$1$ and~$2$ with the $Control$ node
having arbitrarily smaller weight than the other nodes in the gadget.
To achieve so we design a \emph{leveraging gadget} that is internally used in the
circuit-computing gadget and is presented in Section~\ref{s:leverage}.
This gadget reduces the influence of a node with large weight to a node with small weight.
The \emph{leveraging gadget} is also used in the gadgets that we present
subsequently and constitutes one of the key reasons that \nmc{} is PLS-complete. 

\begin{figure}
    \centering
    \includegraphics[scale = 0.8]{figures/Architecture.jpg}
    \caption{The construction of the \nmc{} instance}
\label{f:construction}
\end{figure}

We now present the general construction of the instance of \nmc{} for a given circuit $C$
of the \cf{} problem. Th construction is depicted in Figure~\ref{f:construction}
and we initially discuss the role of each separate gadget. The construction of each separate gadget is presented in the respective section in Appendix.
At first $C_1,C_2$ are circuit-computing gadgets of Figure~\ref{f:CGadget}.
Given the circuit $C$ of the instance of the \cf{}
with $n$-input gates and $m$-output gates
representing the value of the input string. We consider a circuit with
$n+m$ output gates in which the first $n$ gates compute a strictly improving
neighbor solution of the input string if such exists
and otherwise output the input solution.
The last $m$ output gates compute the value of input.
The circuit-computing gadgets $C_1,C2$ simulate the above presented circuit. 
The nodes in $Next1,Next2$ are the output nodes that represent the better
neighbor solution of the inputs $I_1,I_2$ respectively. The nodes in
$Val_1,Val_2$ are also output nodes that represent
the value of each input. The primary role of the \emph{Comparator}
gadget is to compare the values of $I_1,I_2$ and output $1$ if $Val_1 \geq Val_2$.
The result of this comparison is \emph{stored} in the value 
of the $flag$ node. If $flag = 1$ 
then $I_1$ \emph{writes} her better neighboring solution to $I_2$ (respectively when $flag = 0$).
Intuitively if this happens 
then 
in the next \emph{cycle} $I_2$ will have a better value
and will write her improving solution to $I_1$. This goes on and on until no better
neighbor solution exists and both $I_1$ and $I_2$ have the same values. 

We next describe the role of the \emph{Copy} gadgets that may seem quite complicated.
The Copy2 gadget (respectively for Copy1) is responsible for writing $Next1$ to $I_1$ when
$flag = 1$ (respectively when $flag = 0$). If this is the case, the Copy2 gadget creates bias to
$T_2$ and to $I_2$ towards adopting the value of $Next1$.
The reason that we cannot directly copy $Next1$ to $I_2$ is that if $Control2=1$ then $I_2$
may not be willing to adopt the value of $Next1$ due to the values of her neighbors in the
$C_2$ gadget. This problem is fixed with the $T_2$ node. If $flag =1$ then $T_2$ takes the value
of $Next1$ due to the bias of the Copy2 gadget. In case $I_1 \neq Next1$ then the
equality gadget turns the value of the $Control2$ to $0$. Then due to Case~$2$ of
Lemma~\ref{l:SY_gadgets}, $I_2$ has $0$ bias from her
neighbors in $C_2$ and adopts the value of $Next1$ due to the bias of the Copy2 gadget
towards this value. As a result the value of $Next1$ is transferred to $I_2$.


\\
\\
\noindent \textbf{Fixing the Feedback problem}
\\
\\
In the previous paragraph we provided an \emph{ideal} way on how the gadgets behave. As already mentioned
it is easy to design an instance of the \nmc{} in which at any equilibrium the values of the output nodes
are a specific boolean function of the values of the input nodes. However when the \enquote{output nodes} of a gadget
are simultaneously the \enquote{input nodes} of another gadget, the correctness of the 
output nodes is not assured and the feedback problem arises.
Up next we exhibit how consistency is restored in the construction of Figure~\ref{f:construction}.
The \emph{red marks} denote that at any equilibrium of the overall instance of Figure~\ref{f:construction}, the bias of the node due to its participation in this gadget is dominated by the bias of some other gadgets. In other words a \emph{red mark} denotes that the equilibrium value of this node
is indifferent to the values of the internal nodes in this gadget. For example the \emph{red marks} between the $Flag$ and the Copy gadgets denotes that equilibrium value of the $Flag$ node is only determined by the values in internal nodes of the Comparator gadget.
Up next we present how select the weights of the internal nodes of each gadget in order to establish these marks. The exact values of the weights can be found in the Appendix 

The \emph{red mark} between $Control2$ and the $C_2$ gadget denotes that
the equilibrium value of $C_2$ is only determined by the values of the
$Control2$ 's neighbors participating in the equality gadget.
We enforce the latter
by taking the minimum weight of the internal nodes in the equality gadget sufficiently larger than $w_{Control2} >0$ 
(remember that by Lemma~\ref{l:SY_gadgets} the bias of $Control2$ towards the $C_2$ gadget is $w_{Control}$).
This selection guarantees that
at any equilibrium point
$Control2 = (I_2  = Next1)$ no matter the equilibrium values of the $Control2$ 's neighbors in the $C_2$ gadget.
This is formally stated in Lemma~\ref{c:consistent1} that is proven in Section~\ref{s:control} where the exact weights of the nodes
of each gadget are presented.
\begin{replemma}{c:consistent1}
Let an equilibrium of the overall \nmc{} instance of Figure~\ref{f:construction}. Then 
\begin{itemize}
    \item $Control1 = (T_1  =  Next1)$
    \item $Control2 = (T_2  =  Next2)$
\end{itemize}
\end{replemma}
Now consider the red marks between nodes $I_2,T_2$ and the equality gadget. In the high level description of the reduction the value of $Next1$ is copied to $I_2$ as follows: If $flag = 1$ then $T_2$ takes the value of $Next1$. If $I_2 \neq T_2$ then $Control2 = 0$ and then
$I_2$ takes the value of $Next1$ due to the bias of the Copy2 gadget. This analysis disregards the fact that $I_2,T_2$ act as input nodes in the equality gadget and thus may not confront with the bias of Copy2. This potential inconsistency in the values of $I_2,T_2$ with the \enquote{suggested values} of the Copy2 gadget,
is easily fixed by selecting the weights of the internal nodes in Copy2 sufficiently larger than the maximum weight in the equality gadget. In other words the bias of $I_2,T_2$ with respect to Copy2 is huge in comparison with the respective bias of the equality gadget. This \emph{red mark} is formally stated Lemma~\ref{l:copy2}
that is proven in Section~\ref{s:copy} where the weights of the nodes in Copy gadgets are presented. More precisely in Lemma~\ref{l:copy2} we prove that
at any equilibrium of the overall \nmc{} instance of Figure~\ref{f:construction}.
\begin{itemize}
    \item If $Flag = 1$ then $T_2 = Next1$ 
    \item If $Flag = 1$ and $Control2 =0$ then $I_2 =  Next1$
\end{itemize}

\begin{remark}\label{r:remark3}
In case of $I_2$ the extra condition $Control2 = 0$
is needed to ensure that $I_1$ has $0$ bias towards $C_2$ gadget.
The bias of Copy2 is huge in comparison with bias of the equality gadget, but not necessarily with the bias of $C_2$.
\end{remark}


Finally the \emph{red marks}
between the $Flag$
and the Copy gadgets indicate
that $Flag$ takes the output of the \emph{Comparator} gadget. These marks are more tricky to establish. The reason is that both the \emph{Comparator} and the Copy gadgets have input nodes in $Next1, Next2, Val_1, Val_2$ which have weights of the same order of magnitude as output nodes of the circuit-computing gadgets. As a result, this time the weights of the internal nodes in the Comparison gadget cannot be selected sufficiently larger than the respective weights of the Copy gadgets. The bias of the $Flag$ with respect to the Copy gadgets could be easily made negligible to the respective bias of
the Comparator by connecting the $Flag$ with the Copy gadgets with edges of sufficiently small weight.
This is the second point where the absence on weights on the edges plays a major role. We overcome this difficulty by using again the \emph{leveraging gadget} internally in the Copy gadget. Now the \emph{leveraging gadget}
decreases the influences of the internal nodes of the Copy gadgets to the
$Flag$ making its bias much smaller than the bias of the \emph{Comparator}. In Lemma~\ref{l:comparator} we prove that at any equilibrium of the overall \nmc{} instance of Figure~\ref{f:construction}, $Flag$ follows the output of the \emph{Comparator} gadget.

To summarize the above discussion. The \emph{red marks} solve the \emph{Feedback Problem} i.e. at any equilibrium in which $Flag= 1$, $I_2 = Next1$ (respectively when $Flag = 0$). Moreover the $Flag$ node follows the output of the Comparator gadget i.e. $Flag = 1$ if and only if the value of $I_1$ is greater than the value of $I_2$.
\\
\\
\noindent \textbf{Correctness of the Output Nodes}
\\
\\
In the previous paragraphs we have discussed how the \emph{Feedback problem} is solved in our reduction. Informally speaking we select the weights of the nodes in the gadgets in the following order of magnitude
$w_{Control} << w_{\text{equality gadget}} << w_{Copy  gadgets} \sim w_{\text{Comparator}} $
(see also Sections~\ref{s:computing_gadgets}~\ref{s:control}~\ref{s:copy}~\ref{s:comparison_gadget} in Appendix for the exact weights). Unfortunately
this selection creates another serious problem:
The nodes in $Next2, Val_2$ are output nodes of the circuit-computing gadget $C_1$ (respectively for $Next1,Val_1$). By Case~$1$ of Lemma~\ref{l:SY_gadgets} these nodes have bias $\epsilon$ to adopt the output values of the simulated circuit, but this bias $\epsilon$ is very small i.e.
$\epsilon<< w_{Control} << w_{\text{Copy gadgets} } \sim
w_{\text{Comparator} }$. The latter implies that
at an equilibrium of the overall instance of Figure~\ref{f:construction},
the values of $Next2,Val_2$ are not guaranteed to be correct even if $Control_2 = 1$. The latter implies that the nodes in $Next2,Val_2$ may select their values according to the \emph{heavily weighted neighbors} in the Copy and the Comparator gadgets.

The correctness in the values of the nodes $Next2,Val_2$ is ensured
by the design of the \emph{Copy} and the \emph{Comparator} gadgets. 
Apart from their primary role these gadgets are specifically designed to
cause $0$ bias to the outputs nodes of the circuit-computing gadget in which
the better neighbor solution is written. This $0$ unbiases of the output nodes in $C_2$ with their neighbors outside the $C_2$ gadget
in case $Flag = 1$ ($Next1$ is written in $I_2$)
are denoted by the \emph{green marks}
in Figure~\ref{f:construction_1}.
These additional marks are
\emph{conditional} in the sense that their position changes according to the value
of the $Flag$.
Moreover they are \enquote{stronger} than the \emph{red marks}: a \emph{green mark}
from a node to a gadget denotes that at any equilibrium the total weight of its neighbors in this gadget that play $1$ equals the weight of its neighbors that play $0$. The crucial thing to understand is that these \emph{green marks}
guarantee the correctness of the values of the nodes
$Next2,Val_2$ when
$Flag = 1$ because these nodes will play according to the right output of the simulated circuit (Case~$1$ of Lemma~\ref{l:SY_gadgets}). The exact same hold for $Next1,Val_1$ when $Flag = 0$.

\begin{figure}
    \centering
    \includegraphics[scale= 0.4]{figures/ArchFlag1.jpg}
    \caption{Since $flag = 1$ any internal node of the $C_2$ gadget has $0$ bias towards all the other gadgets. As a result, Lemma~\ref{l:SY_gadgets} applies.}
\label{f:construction_1}
\end{figure}

The \emph{green mark} between the nodes
in $Next_2$ and the Copy1 gadget when $flag = 1$ is established by the construction of the Copy gadgets
and is formally stated in Lemma~\ref{l:copy2} that describes the behavior the Copy gadgets (Lemma~\ref{l:copy2}) holds symmetrically
when $flag =0$. The construction of the Copy gadgets and the proof can be found in Section~\ref{s:copy}.

\begin{replemma}{l:copy2}
At any equilibrium point of the \nmc{} instance of Figure~\ref{f:construction} in which $Flag=1$:
\begin{enumerate}
        \item $T_2 = Next1$
        
        \item If $Control2 = 0$ then $I_2 = Next1$
        
        \item $Next2$ has $0$ bias with respect to the Copy1 gadget.
        
    \end{enumerate}
\end{replemma}
\noindent Case~$1$ and~$2$ have been already been discussed in the \emph{Feedback problem}. Case~$3$ 
establishes the \emph{conditional green mark}
between $Next2$ and $Copy1$ when $flag = 1$ (respectively 
for $Next1$ and $Copy2$ when $flag = 0$)

The \emph{green mark} between the nodes in $Val_2$ and the \emph{Comparator} gadget when $flag = 1$ (respectively
for $Val_1$ when $flag =0$) are formally stated in Case~$1$ of Lemma~\ref{l:comparator} and it is established
by the construction of the \emph{Comparator} presented in Section~\ref{s:comparison_gadget}.
We can now establish the correctness of the values of nodes in
$Next2,Val_2$ at any equilibrium with $Flag = 1$.
By Case~$1$ of Lemma~\ref{l:comparator} together with Case~$3$ of Lemma~\ref{l:copy2}
all internal nodes of $C_2$ have $0$ bias towards the remaining gadgets (Figure~\ref{f:construction_1}). Moreover $Flag = 1$ implies that $I_2 = Next1$ and thus $Control2 = 1$.
Now Case~$1$ of Lemma~\ref{l:SY_gadgets} and the fact that all internal nodes of $C_2$ have $0$ bias towards the remaining gadgets imply that $Next2,Val_2$ have the values of the simulated-circuit with input $I_2$.

Up next we deal with the correctness of the values of nodes in $Val_1$ and $Next11$ when $Flag =1$.
We remind that even if at such an equilibrium, $Control1=1$ we could not be sure about the correctness
of the values of these nodes due to their neighbors in the Copy2 and the \emph{Comparator} gadget (Lemma~\ref{l:SY_gadgets} does not apply).
How can we be sure about the correctness of nodes in $Next1,Val_1$ when $Flag = 1$?
This last problem is fixed again by the \emph{Comparator} gadget and here comes its third crucial role.
The \emph{Comparator} also checks whether the nodes in $Next_1$ have correct values with respect to the input $I_1$ and
if it detects incorrectness it outputs $0$ i.e. when $flag = 1$ the correctness of $Next1$ is guaranteed
by the design of the \emph{Comparator} and not by application of Lemma~\ref{l:SY_gadgets}!
This idea was first developed in \cite{SY91} and it as adopted in the subsequent reductions \cite{ET11,GS10}. Our \emph{Comparator} is able to
determine the correctness of the nodes $Next1$ by taking as inputs some internal nodes of the circuit computing gadget (in \cite{SY91} these nodes are referred as control nodes and should not be confused with the $Control$ node of the circuit-computing gadget). The edges between the $C_1,C_2$ and the \emph{Comparator} in Figure~\ref{f:construction_1} illustrate this fact.
In \nmc{} problem designing the \emph{Comparator} gadget is a challenging task
since in
the construction
of the
original \emph{Comparator} gadget crucially uses exponentially small weights on the connecting edges \cite{SY91}. Overcoming the lack of weights on the edges is the final technical contribution of ours. To overcome this difficulty our \emph{Comparator} only guarantees the correctness of the nodes in $Next1$ and not of the nodes in $Val_1$. This is a major difference with the respective \emph{Comparator} gadgets in the previous reductions that ensured correctness both to the nodes in $Next_1, Val_1$. Surprisingly we were able to guarantee that our \emph{Comparator} outputs $1$ ($flag = 1$) if
and only if the \emph{real value} of $I_1$ is greater than the \emph{real value} of $I_2$ even if the nodes in $Val_1$ have incorrect values!
By the term \emph{real value} of $I_1$ we mean the binary string that the simulated circuit $C$ outputs with input $I_1$. We denote this string with $Real-Val(I_1)$. Lemma~\ref{l:comparator} formalizes the above discussion and its proof can be found in Section~\ref{s:comparison_gadget}.

\begin{replemma}{l:comparator}
At any equilibrium of the \nmc{} instance of Figure~\ref{f:construction} in which $flag = 1$ and $Control2 = 1$:

\begin{enumerate}
    \item All the nodes of $C_2$ have $0$ bias to the \emph{Comparator} gadget.
    
    \item The nodes in $Next1$ have the correct value, $Next1 = Real-Next(I_1)$
    
    \item If $Val_2 = Real-Val(I2)$ and $Next1 = Real-Next(I_1)$
    then $Real-Val(I_1) \geq  Real-Val(I_2)$
\end{enumerate}
\end{replemma}
\noindent Case~$1$ of Lemma~\ref{l:comparator} states that when $Next1$ is written to $I_2$
all the nodes in $C_2$ have zero bias towards the \emph{Comparator} gadget (\emph{green marks} in Figure~\ref{f:construction_1}). We remind that the nodes in $Val2$ are \emph{not the only} nodes of $C_2$ that are connected to the \emph{Comparator} gadget. Case~$2$ of Lemma~\ref{l:comparator} establishes the correctness of the nodes in $Next1$ when $flag = 1$ and we remind again that the correctness of the nodes in $Val_1$ is not established (it may be $Val_1 \neq Real-Val(I_1)$). Finally, Case~$3$ states that if the values of the nodes in $Val_2$ are correct then the result of the \emph{Comparator} ($Real-Val(I_1) \geq Real-Val(I_2)$) even if the nodes in $Val_1$ do not have correct values.

\begin{theorem}\label{t:main_max_cut}
The \nmc{} is PLS-complete.
\end{theorem}
\begin{proof}
For a given circuit $C$ of the \cf{}, we can construct in polynomial time the instance of \nmc{} of Figure~\ref{f:construction}. We remind that in the simulated circuit of the circuit-computing gadgets $C_1,C_2$ if for an input string there is
no neighbor string with greater value then the circuit copies the string in its first $n$ output gates. We prove that for
at any equilibrium of \nmc{} of Figure~\ref{f:construction}, $I_1 = Real-Next(I_1) = I_2$ which means that the values of the input nodes in $I_1$ is a solution for the \cf{}.

Let us consider an equilibrium of the \nmc{} of Figure~\ref{f:construction}. Without loss of generality we assume that $flag = 1$.
We first prove that $I_2 = Next1$. Let us assume that $I_2 \neq Next1$. By Lemma~\ref{c:consistent1} we have that $Control2 = 0$. The latter means that Case~$2$ of Lemma~\ref{l:copy2} applies and $I_2 = Next_1$ which is a contradiction.

Since $I_2 = Next1$, by Lemma~\ref{c:consistent1} we have that $Control2 = 1$. Moreover by Case~$3$ of Lemma~\ref{l:copy2}
and Case~$1$ of Lemma~\ref{l:comparator} we have that all nodes of $C_2$ have $0$ bias to the Copy1 and the Comparator gadgets. As a result, Case~$1$ of Lemma~\ref{l:SY_gadgets} applies which means that $Val_2$ and $Next2$ have correct output values i.e. $Val2 = Real-Val(I_2)$ and $Next2 = Real-Next(I_2)$.

By Case~$2$ and~$3$ of Lemma~\ref{l:comparator} we have that
$Real-Val(I_1) \geq Real-Val(I_2)$. As a result, we have that 
\begin{eqnarray*}
Real-Val(I_1) &\geq& Real-Val(I_2)\\
&=& Real-Val(Next1)\\
&=& Real-Val\lp( Real-Next(Next1) \rp)
\end{eqnarray*}
But if $I_1 \neq Real-Next(I_1)$ then $Real-Val(I_1)  > Real-Val\lp( Real-Next(Next1) \rp)$ which is a contradiction.
Thus $I_1 = Real-Next(I_1) = I_2$.
\end{proof}



==> prelim.tex <==
\section{Preliminaries}


%\noindent - For a problem instance  $(S,f, N)$ of $\Pi_{LS}$, algorithm $A$ returns a solution $s\in S$.
%
%\noindent - For a problem instance   $(S,f, N)$ of $\Pi_{LS}$ and a solution $s\in S$, algorithm $B$ decides whether s is a local optimum and, if this is not the case, it returns a neighboring solution with better cost.

We first define three local search problems, i.e., problems where the goal is to find a solution which is locally optimal with respect to the values of all other solutions in its neighborhood.

\noindent \textbf{Local-Max-Cut.}
An instance of \mc{} consists of an edge-weighted graph $H(N,A)$, where $N$ is the set of nodes and $A$ is the set of edges. The weight of edge $a\in A$ is denoted by $w_a$. A \emph{cut} of $H$ is a subset $S\subseteq N$. The \emph{weight} of a cut $S$ is the sum of the weights of the edges crossing it, i.e., $W(S)=\sum_{a\in C(S)}w_a$, where $C(S)=\big\{\{u,v\}\in A: u\in S\,\,and\,\, v\in N\setminus S%] \,\,or\,\,[v\in S\,\, and\,\, u\in N\setminus S]
\big\}$. The \emph{neighborhood} of a cut $S$ is the set $ND(S)$ that contains exactly all the cuts that can be obtained by moving one node from $S$ to $N\setminus S$ or one node from $N\setminus S$ to $S$. A maximal cut is a cut $S$ such that $W(S)\geq W(S')$, for all $S'\in ND(S)$. Given an edge-weighted graph $H$, \emph{\lmc{ }}is the problem of finding a maximal cut of $H$. 

\smallskip
\noindent \textbf{Local-Node-Max-Cut.}
A special case of \mc{} is that of \emph{\nmc{}} where  each node $i\in N$ has some weight $w_i$ and the weight of edge $a=\{i,j\}$ is then $w_{a}=w_iw_j$. In such a case we denote \lmc{ }by \lnmc{}. We work with this definition in Section \ref{sec:wcgsOverview}.

Alternatively, \lnmc{} consists of an (unweighted) undirected graph $H(N,A)$, where $N$ is the set of nodes and $A$ is the set of edges. Each node $i \in N$ is a selfish agent and has a non-negative weight $w_i \geq 0$. Each node selects as value either $0$ or $1$ so as to minimize her cost, which is defined to be the total weight of her neighbors that play the same value. A $0$-$1$ vector $v = (v_1,\ldots,v_{|N|})$ is
a Nash Equilibrium if and only if for all nodes $i \in N$,
\[\sum_{j \in N_i : v_i = v_j}w_j \leq \sum_{j \in N_i : v_i \neq v_j}w_j,\]
where $N_i$ denotes the set of nodes 
that share an edge with node $i$.
In \lnmc{} the goal is to compute a $0$-$1$ vector that is a Nash Equilibrium. We work with this definition in Section \ref{sec:nMCoverview}.

To see the equivalency of the two definitions observe that \[\sum_{j \in N_i : v_i = v_j}w_j \leq \sum_{j \in N_i : v_i \neq v_j}w_j\Leftrightarrow \sum_{j \in N_i : v_i = v_j}w_iw_j \leq \sum_{j \in N_i : v_i \neq v_j}w_iw_j,\] i.e., $i$ is at her best response iff the weight of the cut only decreases if $i$ switches sides. 

We also care about approximate equilibria.
In the same context and for any $a\geq1$, a $0$-$1$ vector $v = (v_1,\ldots,v_{|N|})$ is
an $a$-approximate equilibrium if   for all nodes $i \in N$,
\[\sum_{j \in N_i: v_i = v_j}w_j \leq a \cdot\sum_{j \in N_i: v_i \neq v_j}w_j.\]


\smallskip\smallskip\noindent \textbf{Circuit-Value with  Flip-Neighborhood.}
The very first problem proved to be PLS-complete is \emph{\cf{}}, where an instance consists of a boolean circuit
$C$ with $n$ input gates, $m$ output gates and (wlog) only NOR gates. The \emph{value $C(I)$} of an $n$-bit input string $I$
is the integer corresponding to the $m$-bit (binary) string in the output gates. Given  a circuit $C$, \cf{} searches for a string $I$ for which the value of the circuit 
cannot increase if we flip any of $I$'s bits, % the value of the produced string does not increase, 
i.e. for all $I'$ with Hamming distance $1$ from $I$, $C(I)\geq C(I')$. Strings with Hamming distance $1$ are called \emph{neighbors}.

\smallskip Next, we move on to give some Complexity Theory related preliminaries.\\
\noindent \textbf{Local Search Problems.} An instance of a \emph{local search problem} is a triple   $(S,f, N)$, where $S$ is the set of \emph{feasible solutions} (or simply \emph{solutions}) of a combinatorial optimization problem, $f:S\rightarrow \mathbb{R}$ is a \emph{cost} function for the solutions in $S$ and  $N:S \rightarrow 2^S$ is a \emph{neighborhood} function on $S$ returning for each $s\in S$ the set of its neighboring feasible solutions.

A \emph{local search problem} $\Pi_{LS}$ is specified by a set of local search problem instances and it is either a minimization or a maximization problem. The problem is to find for any given instance  $(S,f, N)$  a locally optimal solution $s^*\in S$, i.e., an $s^*\in S$ so that $f(s^*)\leq f(s)$ for a minimization problem or $f(s^*)\geq f(s)$ for a maximization problem. Examples of local search problems are \lmc{} and \lnmc{} defined below.


\smallskip\noindent \textbf{Polynomial-time Local Search (PLS).} The \emph{class NPO} consists of combinatorial optimization problems for which we can decide in polynomial time whether an input $x$ defines a correct problem instance, for which the cost function is computable in polynomial time, and for which it is decidable in polynomial time whether a string $s$ defines a feasible solution, where the size of each feasible solution is polynomially bounded in the input size.

Let $\Pi_{LS}$ be a local search problem and let $\Pi$ be the underlying combinatorial optimization problem. Local search problem $\Pi_{LS}$ is in the \emph{class PLS} (Polynomial-time Local Search) if $\Pi\in NPO$ and if two polynomial-time algorithms $A$ and $B$ exist that satisfy the following properties:
\begin{itemize}
\item For a problem instance  $(S,f, N)$ of $\Pi_{LS}$, algorithm $A$ returns a solution $s\in S$.
\item For a problem instance   $(S,f, N)$ of $\Pi_{LS}$ and a solution $s\in S$, algorithm $B$ decides whether s is a local optimum and if this is not the case, it returns a neighboring solution with better cost.
\end{itemize}


\smallskip\noindent \textbf{PLS Reductions and Completeness.} Local search problem $\Pi_{LS}$ is \emph{PLS-reducible} to local search problem
$\Pi'_{LS}$,  if two polynomial-time algorithms $\phi_1$ and $\phi_2$ exist that
satisfy the following properties:

\begin{itemize}
\item Algorithm $\phi_1$ transforms a problem instance $I$ of $\Pi_{LS}$ into a problem instance
$\phi_1(I)$ of  $\Pi'_{LS}$.
\item Algorithm $\phi_2$ maps a problem instance $I=(S,f,N)$ of $\Pi_{LS}$ and a solution
$s'\in S'$  with  $\phi_1(I)=(S',f',N')$  to a solution $s\in S$.
\item For a problem instance $I$ of $\Pi_{LS}$, we have that if $s'\in S'$ is a local optimum for
$\phi_1(I)=(S',f',N')$, then $\phi_2(I,s')$  is a local optimum for $I$.
\end{itemize}

Note that  if local search problem $\Pi_{LS}$ is PLS-reducible to local search problem $\Pi'_{LS}$, then the existence of a polynomial-time algorithm for $\Pi'_{LS}$ implies the existence of  a polynomial-time algorithm for $\Pi_{LS}$. In other words, $\Pi'_{LS}$ is at least as hard as $\Pi_{LS}$.
Additionally, PLS-reductions are transitive, which means that if $\Pi_{LS}$ is PLS-reducible to $\Pi'_{LS}$ and $\Pi'_{LS}$ is PLS-reducible to $\Pi''_{LS}$, then $\Pi_{LS}$ is also PLS-reducible to $\Pi''_{LS}$.

To capture the hardest problems of the class we define \emph{PLS-completeness}. A local search problem is \emph{PLS-hard} if  each problem $\Pi_{LS} \in PLS$ is PLS-reducible to it. By the above discussion, to prove that a local search problem $\Pi_{LS}$ is PLS-hard it suffices to reduce a PLS-hard problem to it. A local search problem is \emph{PLS-complete} if it is in PLS and is PLS-hard.  Sch\"affer and Yannakakis  \cite{SY91} have  proved that \lmc{} is  PLS-complete (see \cite{MA10} for a survey), which directly implies that \lnmc{} is in PLS.

\smallskip
Next, we move on to give some Game Theory related  preliminaries.

\noindent 
 \textbf{Weighted Congestion Games.} A \emph{Weighted Congestion Game} consists of $n$ weighted players each having a positive weight $w_i$, a set of resources $E$ together with a non-decreasing latency function  $\ell_e:\mathbb{R}_{\geq0}\rightarrow \mathbb{R}_{\geq0}$ for each resource $e\in E$, and a non-empty strategy set $S_i\subseteq 2^E$ for every player $i\in [n]$, where $[n]=\{1,\ldots,n\}$.  A subclass of Weighted Congestion Games is that of \emph{Weighted Network Congestion Games} where there is an underlying (undirected) network with some of the vertices forming origin-destination pairs. The  resources of the game are
the links of the network. Each  player $i$ is assigned to some origin-destination pair $o_i$-$d_i$ and her strategy set consists of all the $o_i$-$d_i$ paths.  Formally, a Weighted Network Congestion Game is a tuple $\mathcal{G}=\big(G(V,E),(c_e)_{e\in E},(w_i)_{i\in [n]},((o_i,d_i))_{i\in [n]}\big)$.
%
In the special case where all players share a common origin-destination pair  we have a single-commodity game, else we have a multi-commodity game. 

\smallskip
\noindent \textbf{Configurations, Costs and Equilibria.} 
Player i chooses a strategy $s_i$ in her strategy set $S_i$ (an $o_i$-$d_i$ path for network games). All these choices combined form a configuration. Formally, a \emph{configuration} is a vector $(s_1,\ldots,s_n)$, with $s_i\in S_i$. In order to capture single player deviations, given an initial configuration $s=(s_1,\ldots,s_n)$ we denote by $(s_i',s_{-i})$ the configuration where player $i$ has changed her strategy from $s_i$ to $s_i'$ while all other players play according to $s$, i.e., player $j\neq i$ chooses
$s_i$. Under a configuration $s=(s_1,\ldots,s_n)$ each resource gets some \emph{congestion} $x_e$ equal to  the sum of the weights of the players choosing it, i.e., $x_e=\sum_{i:e\in s_i}w_i$, and has \emph{cost} $\ell_e(x_e)$. Player i's \emph{cost} under configuration $s$ is   
$c_i(s)=\sum_{e\in s_i}\ell_e(x_e)$. A configuration $s$ is a \emph{Nash equilibrium} if no player has an incentive to deviate. Formally, $s$ is a Nash equilibrium if $\forall i\in [n],\forall s'_i\in S_i:c_i(s)\leq c_i(s'_i,s_{-i})$. Instead of Nash equilibrium we may simply say \emph{equilibrium}.


==> wCGsoverview.tex <==
\section{Computing Equilibria in Weighted Congestion Games}

\label{sec:wcgsOverview}
In this section we state and provide proof sketches for our PLS-completeness theorems. In the first part we do so for single-commodity Weighted Network Congestion Games on series parallel networks with linear latencies (Theorem \ref{thm:sepaPLShard}) and in the second part we do so for multi-commodity Weighted Network Congestion Games with the identity function on all links (Theorem \ref{thm:mutiPLS}). For the complete proofs see sections \ref{sec:singlePLS} and \ref{sec:multiPLS} respectively.

\bigskip
\noindent\textbf{Single-Commodity Weighted Network Congestion Games.}\\
We prove that it is PLS-hard to compute an equilibrium of a Weighted Congestion Game, even if it is a Weighted Network Congestion Game on a series-parallel single-commodity network with linear latencies, i.e., with latency functions of the form $\ell_k(x)=a_kx$.
We do so by reducing from \lmc. 

\begin{theorem}\label{thm:sepaPLShard}
Computing a Nash equilibrium in single-commodity Weighted Network Congestion Games with linear latency functions is PLS-complete.
\end{theorem}


\begin{proof}[Proof sketch]
We will reduce from the PLS-complete problem \lmc{}. Given an instance of \lmc{} we will construct a Weighted Network Congestion Game for which the Nash equilibria will correspond to maximal solutions of \lmc{} and vice versa. 

To give the construction, let $H(N,A)$ be an edge-weighted graph of a \lmc{} instance and let $n=|N|$ and $m=|A|$. In the constructed Weighted Network Congestion Game  instance there will be $3n$ players which will share $n$ different weights inside the set $\{16^i:i\in [n]\}$ so that for every $i\in[n]$ there are exactly 3 players having weight $w_i=16^i$.  All  players share a common origin-destination pair $o-d$ and choose $o-d$  paths on a series-parallel graph $G$.
%
Graph $G$ is a parallel composition  of two identical  copies of a series-parallel graph.We call these copies $G_1$ and $G_2$. In turn, each of $G_1$ and $G_2$ is a series composition of $m$ different series-parallel graphs, each of which corresponds to the $m$ edges of $H$. For every $\{i,j\}\in A$ let $F_{ij}$ be the series-parallel graph that corresponds to edge $\{i,j\}$. $F_{ij}$ is presented in Fig. \ref{fig:sepaPLS}, where $D$ is assumed to be a (polynomially) big enough constant. An example graph $G$ is given in Fig. \ref{fig:sepaExample}. 

\begin{figure}
    \centering
    \includegraphics[scale=0.1]{sepaPLS.png}
    \caption{The series-parallel network $F_{ij}$ that corresponds to edge $\{i,j\}\in A$}
    \label{fig:sepaPLS}
\end{figure}



Observe that in each of $G_1$ and $G_2$ there is a unique  path that contains all the links with latency functions $\ell_i(x)$, for $i\in[n]$, and call these paths $p^u_i$ and $p_i^l$ for the upper ($G_1$) and lower ($G_2$) copy respectively. Note that each of $p^u_i$ and $p_i^l$ in addition to those links, contains some links with latency function of the form $\frac{w_{ij}x}{w_iw_j}$. These links for path $p^u_i$ or $p_i^l$ are in one to one correspondence to the edges of node $i$ in $H$  and this is crucial for the proof.

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{sepaExample.jpg}
    \caption{An example of the structure of the construction for a graph $H(N,A)$, with $N=\{1,2,3,4\}$ and $A=\{\{1,2\},\{1,3\},\{1,4\},\{2,4\}\}$. %For ease of notation we have not included the latency functions.
    Each of the  upper and lower parts consists of  copies of $F_{12}$, $F_{13}$, $F_{14}$ and $F_{24}$ connected in series.}
    \label{fig:sepaExample}
\end{figure}

By the choice of the players' weights and the latency functions' slopes, one can show  that at a Nash equilibrium, a player of weight $w_i$ chooses either $p^u_i$ or $p_i^l$. %and,  additionally, $p^u_i$ and $p_i^l$  will each have  at least one player (of weight $w_i$). %This mainly happens because a player of weight, say, $w_k$   sees an overall weight load on her path of the same order to her weight even if all players with weight $\leq w_k$ are on her path ( $3\sum_{l=1}^{k}16^l=\frac{16^{k+1}-1}{16-1}$).
The formal proof uses induction starting from larger weights. The heaviest players, i.e., players with weight $w_n$, have a dominant strategy to choose either $p^u_n$ or $p_n^l$ since $\ell_n(x)$ has a significantly smaller slope  than all other $\ell_i(x)$'s, small enough so that even if all other players choose the same paths (reaching a load of at most $3\sum_{l=1}^{n}16^l=\frac{16^{n+1}-1}{16-1}$ ), still players of weight $w_n$ prefer $p^u_n$ or $p_n^l$ over all other paths. But then, $p^u_n$ and $p_n^l$  get a lot of weight load at equilibrium compared to the weight of lighter players. This makes the links on these paths look like they get some big additive constants, which makes them extremely expensive for all lighter players and these players exclude them from their strategy space. That said, by the same reasoning, the players of weight $w_{n-1}$ have a dominant strategy to choose either $p^u_{n-1}$ or $p_{n-1}^l$ and this inductively proves true for all $i\in [n]$.


Additionally, one can  prove  that $p^u_i$ and $p_i^l$  will have  at least one player (of weight $w_i$). The underlying idea is that if wlog $p^u_i$  has two players (of weight $w_i$) then the third player of weight $w_i$ prefers to go to $p^l_i$, since it is going to be empty.   %each and thus it is like only one player has the choice of moving from $p^u_i$ to $p_i^l$ or vice versa. 
This already provides a good structure of a Nash equilibrium and players of different weights, say $w_i$ and $w_j$, may go through the same link in $G$ (the edge with latency function $w_{ij}x/w_iw_j$)  only if  $\{i,j\}\in A$. The correctness of the reduction lies in the fact that players in $G$ try to minimize their costs incurred by these type of links  in the same way  one wants to  minimize the sum of the weights of the edges in each side of the cut when solving \lmc. 


Given a maximal solution $S$ of \lmc{} the proof shows that  the configuration $Q$ that for every $k\in S$ routes $2$ players through $p_k^u$ and $1$ player through $p_k^l$ and for every $k\in N\setminus S$ routes $1$ player through $p_k^u$ and $2$ players through $p_k^l$ is an equilibrium. Conversely, given an equilibrium $Q$ the cut $S=\{k\in N:\mbox{2 players have chosen $p_k^u$ at $Q$}\}$  is a maximal solution of \lmc. 

Assume that we are at equilibrium and consider a player of weight $w_k$ that has chosen $p_k^u$ and wlog $p_k^u$ is chosen by two players (of weight $w_k$). By the equilibrium conditions the cost she computes for $p_k^u$ is at most the cost she computes for $p_k^l$,  which  implies
$$\sum_{i=1}^m\frac{2D16^k}{4^k}+\sum_{\{k,j\}\in A}\frac{w_{kj}(2\cdot16^k+x_j^u16^j)}{16^k16^j} \leq \sum_{i=1}^m\frac{2D16^k}{4^k}+\sum_{\{k,j\}\in A}\frac{w_{kj}(2\cdot16^k+x_j^l16^j)}{16^k16^j}$$
where $x^u_j$ (resp. $x_j^l$) is either $1$ or $2$ (resp. $2$ or $1$) depending whether, for any $j:\{k,j\}\in A$, one or two players (of weight $w_j$) respectively have chosen path $p_j^u$. By canceling out terms, the above implies 
\begin{equation}\label{eqn:LmcToEqMain}
\sum_{\{k,j\}\in A}w_{kj}x_j^u \leq \sum_{\{k,j\}\in A}w_{kj}x_j^l\Leftrightarrow \sum_{\{k,j\}\in A}w_{kj}(x_j^u-1) \leq \sum_{\{k,j\}\in A}w_{kj}(x_j^l-1)
\end{equation}

Define $S=\{i\in N:x_i^u=2\}$. By our assumption it is  $k\in S$ and the left side  of (\ref{eqn:LmcToEqMain}), i.e., $\sum_{\{k,j\}\in A}w_{kj}(x_j^u-1)$, is the sum of the weights of the edges of $H$ with one of its nodes being $k$ and the other belonging in $S$. Similarly, the right side of of (\ref{eqn:LmcToEqMain}), i.e., $\sum_{\{k,j\}\in A}w_{kj}(x_j^l-1)$ is the  sum of the weights of the edges with one of its nodes being $k$ and the other belonging in $N\setminus S$. But then  (\ref{eqn:LmcToEqMain}) directly implies  that for the (neighboring) cut $S'$ where  $k$  goes from $S$ to $N\setminus S$ it holds $W(S)\geq W(S')$. Since $k$ was arbitrary (given the symmetry of the problem), this holds for every $k\in [n]$ and thus for every $S'\in ND(S)$ it is  $W(S)\geq W(S')$ proving one direction of the claim. Observing that the argument works backwards the proof completes. %   For the formal proo, to define function $\phi_2$, given the constructed instance and one of its solutions, say $s'$, $\phi_2$ returns  solution $s=\{k\in N:\mbox{2 players have chosen $p_k^u$ at $s'$}\}$. 
\end{proof} 

\smallskip
\noindent\textbf{Multi-Commodity Weighted Network Congestion Games.}\\
We prove that it is PLS-hard to compute an equilibrium in  Weighted Congestion Games, even if it is a Weighted Network Congestion Game with all latency functions equal to the identity function, i.e., for any link $e$, $\ell_e(x)=x$. This result is stronger in some aspect than that of Section \ref{sec:singlePLS} since   we allow only the weights of the players to be exponential. Note that if both the coefficients of the linear latency functions and the weights of the players are polynomial, then best response dynamics converges to an equilibrium in polynomial time. For the proof, we reduce from \lnmc{} which, as we prove in %Section \ref{sec:nodeMaxCut} (
Theorem \ref{t:main_max_cut}, is PLS-complete. 

\begin{theorem}\label{thm:mutiPLS}
Computing a Nash equilibrium in multi-commodity Weighted Network Congestion Games with all links having the identity function as their latency function is PLS-complete.
\end{theorem}

\begin{proof}[Proof sketch.]
We will reduce from the PLS-complete problem \lnmc{}.  For an instance of \lnmc{} we will construct a multi-commodity Network Congestion Game where every equilibrium will correspond to a maximal solution of \lnmc{}  and vice versa. Our construction draws ideas from Ackermann et al. \cite{ARV08}.

Skipping many of the details  (that can be found in Section \ref{sec:multiPLS}), in the constructed instance  for every $i\in [n]$, Player $i$ will essentially have two path choices at equilibrium, say $p^u_i$ and  $p^l_i$, that cost-wise dominate all others.  For any $i,j\in [n]$,   $p^u_i$ and   $p^u_j$ (resp. $p^l_i$ and   $p^l_j$) may have in common only  one link that itself belongs only to them, say link $e_{ij}^u$ (resp. $e_{ij}^l$). These links ($e_{ij}^u$ and $e_{ij}^l$) are present  only if $\{i,j\}$ is an edge of $H$, i.e., $\{i,j\}\in A$, and have the identity function as their latency function. What holds is that for every $i \in [n]$, $p^u_i$'s cost differs from $p^l_i$'s cost only because of the $e_{ij}^u$'s and $e_{ij}^l$'s for the $j$'s neighboring $i$ in $H$.

Assume we are at equilibrium. By the above discussion player $i\in[n]$ may only have chosen $p^u_i$ or $p^l_i$. Let $S=\{i\in [n]: \mbox{player $i$ has chosen $p^u_i$}\}$. The proof shows that $S$ is a solution to \lnmc{}. By the equilibrium conditions for every $i\in S$ the cost of $p_i^u$, say $c_i^u$, is less than or equal to the cost of $p^l_i$, say $c_i^l$. By defining $S_i$ to be the neighbors of $i$ in $S$, i.e. $S_i=\{j\in S:\{i,j\}\in A\}$, and $N_i$ be the neighbors of  $i$ in $N$, i.e. $N_i=\{j\in N:\{i,j\}\in A\}$,  $c_i^u\leq c_i^l$ translates to

$$K+\Big(\sum_{j\in N_i}w_i+\sum_{j\in S_i}w_j\Big)
\leq K+\Big(\sum_{j\in N_i}w_i+\sum_{j\in N_i\setminus S_i}w_j\Big)$$ 

for some big constant $K$ with the costs in the second and fourth parenthesis coming from the $e_{ij}$'s for the different $j$'s. This equivalently gives $$\sum_{j\in S_i}w_j\leq\sum_{j\in N_i\setminus S_i}w_j\Leftrightarrow \sum_{j\in S_i}w_iw_j\leq\sum_{j\in N_i\setminus S_i}w_iw_j.$$ 

The right side of the last inequality equals to the weight of the edges with $i$ as an endpoint that cross  cut $S$. The left side equals to the weight of the edges with $i$ as an endpoint that cross the cut $S'$, where $S'$ is obtained by moving $i$ from $S$ to $N\setminus S$. Thus for $S$ and $S'$ it is $W(S')\leq W(S)$. A similar argument (or just symmetry) shows that if $i\in N\setminus S$ and we send $i$ from $N\setminus S$ to  $S$ to form a cut $S'$ it would again be  $W(S')\leq W(S)$. Thus, for any $S'\in ND(S)$ it is $W(S)\geq W(S')$ showing that  $S$ is a solution to \lnmc{}. Observing that the argument works backwards we have that from an arbitrary solution of \lnmc{} we may get an equilibrium for the constructed Weighted Congestion Game instance.
\end{proof}








\endinput



















We start with the following observation. \nik{we \textit{need} a figure for this way to simulate constants} Since we have a multi-commodity instance we can simulate (exponentially large) constants by replacing a link $\{j,k\}$ with a three link path $j-o_{jk}-d_{jk}-k$, adding a player with origin $o_{jk}$ and destination $d_{jk}$ and weight equal to the desired constant. 
Let $H(N,A)$ be the node-weighted graph of an instance of \lnmc{} and let $n=|N|$ and $m=|A|$. The Weighted Network Congestion Game will have $n$ ``origimal'' players,  with player $i$ having her own origin destination $o_i-d_i$ pair and weight $w_i$ equal to the weight of node $i\in N$. In the constructed network there will be many $o_i-d_i$ paths for every player $i$ but there will be exactly two paths that cost-wise dominate all others. By suitably defining the  the weights of some ``complementary'' players, at equilibrium, every original  player will choose one of the two paths that correspond to her. This choice for player $i$ will be equivalent to picking the side of the cut that node $i$ should lie in order to get a maximal solution of \lnmc{}. 

\begin{figure}
    \centering
    \includegraphics[scale=0.5]{multiPLS2.eps}
    \caption{(a) The construction of the reduction of Theorem \ref{thm:mutiPLS}. As an example, in orange are  the least costly $o_2-d_2$ paths $p_2^u$ (up) and $p_2^l$ (down), each with cost equal to $2D+2d
+(n-2)D$. (b) The replacement of the red node at the $i$-th row and $j$-th column of the upper half-grid whenever edge $\{i,j\}\in A$. A symmetric replacement happens in the lower half-grid.}
    \label{fig:multiPLS}
\end{figure}

The network construction is shown in Fig. \ref{fig:multiPLS}. It has $n$ origins and $n$ destinations. The rest of the vertices lie either on  the lower-left half (including the diagonal) of a  $n\times n$ grid, which we call the upper part, or the upper-left half   of another $n\times n$ grid, which we call the lower part. 
%
To complete the construction, if $\{i,j\}\in A$ (with wlog $i<j$) we replace the (red) vertex at position $i,j$ of the upper and the lower half-grid ($1,1$ is top left for the upper half-grid and lower left for the lower half-grid) with two vertices connected with a link, say $e^u_{ij}$ and $e_{ij}^l$ respectively, with latency function $\ell_{ij}(x)=x$, where the first vertex connects with the vertices at positions $i,j-1$ and $i-1,j$ of the grid and the second vertex connects to the vertices at positions $i+1,j$ and $i,j+1$ (see also Fig. \ref{fig:multiPLS}b). The cost of these links are much smaller than all other links.

%Note that if we take $d\gg \sum_{k\in [n]}w_k$, then,  for any $i\in [n]$, paths $p^u_i$ and $p^l_i$  still have significantly lower  costs  than all other $o_i-d_i$ paths. Additionally, if $\{i,j\}\in A$ then $p^u_i$ and $p^u_j$ have a single common link and $p^l_i$ and $p^l_j$ have a single common link, namely $e^u_{ij}$ and $e_{ij}^l$ respectively,  which add some extra cost to the paths (added to $c_i$ defined above).

Player $i$ will essentially have to path choices, path $p^u_i$ that starts at $o_i$, continues horizontally through the upper part for as much as it can and then continues vertically to reach $d_i$, and path $p^l_i$ which does the exact same thing through the lower part (for an example see Fig. \ref{fig:multiPLS}a). These paths by construction cost-wise dominate all others and $p^u_i$'s cost differ from $p^l_i$'s cost only because of the $e_{ij}^u$'s and $e_{ij}^l$'s for the $j$'s neighboring $i$ in $H$.

Assume we are at equilibrium. By the above discussion player $i\in[n]$ may only have chosen $p^u_i$ or $p^l_i$. Let $S=\{i\in [n]: \mbox{player $i$ has chosen $p^u_i$}\}$. The proof shows that $S$ is a solution to \lnmc{}. By the equilibrium conditions for every $i\in S$ the cost of $p_i^u$, say $c_i^u$, is less than or equal to the cost of $p^l_i$, say $c_i^l$. By defining $S_i$ to be the neighbors of $i$ in $S$, i.e. $S_i=\{j\in S:\{i,j\}\in A\}$, and $N_i$ be the neighbors of  $i$ in $N$, i.e. $N_i=\{j\in N:\{i,j\}\in A\}$,  $c_i^u\leq c_i^l$ translates to 
$$K+\Big(\sum_{j\in N_i}w_i+\sum_{j\in S_i}w_j\Big)\leq K+\Big(\sum_{j\in N_i}w_i+\sum_{j\in N_i\setminus S_i}w_j\Big)$$ 
for some big constant $K$ with the costs in the second and fourth parenthesis coming from the $e_{ij}$'s for the different $j$'s. This equivalently gives $$\sum_{j\in S_i}w_j\leq\sum_{j\in N_i\setminus S_i}w_j\Leftrightarrow \sum_{j\in S_i}w_iw_j\leq\sum_{j\in N_i\setminus S_i}w_iw_j.$$ 

The right side of the last inequality equals to the weight of the edges with $i$ as an endpoint that cross  cut $S$. The left side equals to the weight of the edges with $i$ as an endpoint that cross the cut $S'$, where $S'$ is obtained by moving $i$ from $S$ to $N\setminus S$. Thus for $S$ and $S'$ it is $W(S')\leq W(S)$. A similar argument (or just symmetry) shows that if $i\in N\setminus S$ and we send $i$ from $N\setminus S$ to  $S$ to form a cut $S'$ it would again be  $W(S')\leq W(S)$. Thus, for any $S'\in ND(S)$ it is $W(S)\geq W(S')$ showing that  $S$ is a solution to \lnmc{}. Observing that the argument works backwards we have that from an arbitrary solution of \lnmc{} we may get an equilibrium for the constructed Weighted Congestion Game instance. 
%\end{proof}
